Generative Tweening: Long-term Inbetweening of 3D Human Motions

The ability to generate complex and realistic human body animations at scale, while following specific artistic constraints, has been a fundamental goal for the game and animation industry for decades. Popular techniques include key-framing, physics-based simulation, and database methods via motion graphs. Recently, motion generators based on deep learning have been introduced. Although these learning models can automatically generate highly intricate stylized motions of arbitrary length, they still lack user control. To this end, we introduce the problem of long-term inbetweening, which involves automatically synthesizing complex motions over a long time interval given very sparse keyframes by users. We identify a number of challenges related to this problem, including maintaining biomechanical and keyframe constraints, preserving natural motions, and designing the entire motion sequence holistically while considering all constraints. We introduce a biomechanically constrained generative adversarial network that performs long-term inbetweening of human motions, conditioned on keyframe constraints. This network uses a novel two-stage approach where it first predicts local motion in the form of joint angles, and then predicts global motion, i.e. the global path that the character follows. Since there are typically a number of possible motions that could satisfy the given user constraints, we also enable our network to generate a variety of outputs with a scheme that we call Motion DNA. This approach allows the user to manipulate and influence the output content by feeding seed motions (DNA) to the network. Trained with 79 classes of captured motion data, our network performs robustly on a variety of highly complex motion styles.

==> Long-term 3D Motion Inbetweening/Limitation.tex <==
\subsection{Limitations}
%Our method has the following limitations.
Although our network can interpolate keyframe poses over a much longer time interval than traditional methods, to guarantee the naturalness of the synthesized transition, the maximum allowable time interval between any neighbouring keyframes is still limited by the size of the receptive field of the generator. A possible solution to support even longer time intervals is to do hierarchical synthesis which synthesizes some critical frames first and then generates motions in shorter intervals. Our network operates at a fixed temporal resolution. If two completely different keyframes are specified in a very short interval and their transition is not achievable at the given speed, then one of them may be filtered out as an outlier. 

Our Motion DNA scheme provides a soft control on the style of the output motion. How much it impacts the output style depends on the keyframe constraints. For example, as shown in the supplemental video, when the keyframes and the Motion DNA are both poses from martial arts, the output usually capture the characteristics of martial arts in both arms and legs. However, when the keyframes are walking poses, the result will look less like martial arts, where the output has punching and defending gestures in the upper body but with walking pose in the lower body. Another limitation is that because it uses static representative frames, the Motion DNA contains only the iconic postures of the motion, and might fail to capture the style reflected in the subtle body dynamics. Additionally, in some cases, such as Case 2 in the video, the motions near keyframes can look similar even though different Motion DNAs were provided.

Our method can at times produce foot sliding or skating artifacts, or feet may not properly contact the ground. As we demonstrate in the video for the rigged animation result, these can be fixed by a simple  postprocessing~\cite{li2017auto}. In future work, a loss could be adopted to minimize foot sliding or skating, similar to Holden~et~al.~\shortcite{holden2016deep}: we believe this may be tricky for the CMU dataset we used because there are some dance motions that intentionally use foot sliding.

Some of the generated motions from our method can have overly fast root rotation, such as Case 2 in the video, or be a bit monotonous, such as Case 4 in the video. Future work might address these issues by for example using additional losses.

==> Long-term 3D Motion Inbetweening/additional_features.tex <==

\begin{figure*}
    \includegraphics[width=0.85\textwidth]{fig/path_variation.png}
    \caption{Motion Generation given sparse root coordinates. Two synthesized motion sequences given the same keyframes (position of the root joints as pink dots on the ground) and different representative frames. Top row: the $100$th, $500$th, and $700$th frame from a synthesized sequence. Bottom row: the corresponding frames from another sequence synthesized with a different set of representative frames.}
    \label{fig:root}
\end{figure*}

 \begin{figure*}
    \includegraphics[width=0.6\textwidth]{fig/halfbody.pdf}
    \caption{Motion Generation given random half-body joints. Left: keyframe partial joints inputs and their times. Right: the synthesized 3D poses at keyframes (pink) and nearby frames (blue). }
    \label{fig:halfbody}
\end{figure*}

 \begin{figure*}
    \includegraphics[width=0.85\textwidth]{fig/2D_to_3D.pdf}
    \caption{Motion Generation given manually made 2D poses. Left: 2D keyframe inputs drawn on the x-y plane and their times. Right: the synthesized 3D poses at keyframes (pink) and nearby frames (blue). }
    \label{fig:2D}
\end{figure*}
\section{Additional Features}
In addition to the features discussed above, our method can also be used when only part of the body pose is specified at keyframes. We can change the format of the input (Section \ref{sec:input_sequence_format}) to the network, so that coordinates are only specified at the desired joints and the rest of the joints are masked out in the input matrix during both, training and testing.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Partial Body Control: Root}
Figure~\ref{fig:root} shows the case where only the root joint positions are specified by the user at sparse locations (pink dots on the ground). The two rows show two synthesized sequences generated with the same root joint positions but different representative frames. From left to right, the three frames are the $100$th, $500$th, and $700$th frames. Note that the two generated sequences exhibit different root trajectories and local motions.

\subsection{Partial Body Control: Half-body} 
We trained a network that the keyframe input can contain either the whole body joints or only half of the body's joints. Figure~\ref{fig:halfbody} shows the 3D motion sequences synthesized from partially given keyframe poses.

\subsection{Partial Body Control: 2D Joints} 
Users might want to create 3D skeleton poses by sketching the keyframes in 2D. For this task, we trained a network by providing only the x and y coordinates of the joints and the root. To handle non-standard pose input such as casually drawn stick figures, we trained the network with augmented 2D poses. In Figure \ref{fig:2D}, we show that our network is able to lift the 2D keyframes into 3D and synthesize natural 3D motions. Although the input has stretched and uneven bone lengths, the network manage to synthesize feasible 3D poses that mimic the 2D input. The recent work VideoPose3D~\cite{pavllo:videopose3d:2019} also predicts 3D motion from the 2D motion, but it cannot perform the long-term motion inbetweening task.
%Keyframe control on partial body.
%only give root. Only give 2D joints.




==> Long-term 3D Motion Inbetweening/conclusion.tex <==
\section{Conclusion and Future Work}
We proposed a novel deep generative modeling approach, that can synthesize extended and complex natural motions between highly sparse keyframes of 3D human body poses. Our key insight is that conditional GANs with large receptive field and appropriate input representation are suitable for enforcing keyframe constraints in a holistic way. However, although GANs can generate realistic local motions, they tend to diverge during training for generating global motions. From extensive experiments, we discovered that global motions can be predicted from local motions using neural networks. Thus, we have introduced a two-stage generative adversarial network that first synthesizes local joint rotations and then predicts a global path for the character to follow. 

We also proposed a novel range-constrained forward kinematics layer that helps the network explore a continuous rotation representation space with biomechanical constraints and thus, can produce natural-looking motions. To synthesize different results with the same keyframes, we introduced a new authoring concept, called Motion DNA, which allows users to influence the style of the synthesized output motion.

We compared our method with a closely related work, RTN~\cite{Harvey:2018:Recurrent} and showed superior results for our task. Not only does our method support additional capabilities, our trained deep model also generalizes to RTN's task. Our method handles more complex motions and provides users the flexibility of choosing their preferred sequence among a variety of synthesized results.

In the near future, we plan to train a more flexible system that allows users to control various subsets of joints or specify an arbitrary trajectory. This can be easily achieved by masking out random joints or providing trajectories in the input during training, which is supported by our input format. Another interesting direction is to extend our method to long-term inbetweening of non-human characters. While our current approach is highly efficient and can perform in real-time for short sequences, being able to update extended motion sequences in real-time would enable new possibilities and impact next-generation character animation control systems in gaming and motion planning in robotics.

% Connelly: removed to fit in 13 pages the following:
%, e.g. synthesizing upper body motions given leg motions as input. Our method is general and may not be limited to biped characters.

==> Long-term 3D Motion Inbetweening/experiments_new.tex <==
\section{Experiments and Evaluation}
%We implemented our system using PyTorch~\cite{paszke2017automatic} and 
We conducted various experiments to evaluate the different components of our system. We first evaluated the effectiveness of our Range-Constrained motion representation. We then measured the accuracy of the global path predictor by comparing its results to the ground truth. We also evaluated the local motion generator in two ways: (1) quantitatively, we measured how well the generated motion follows the input keyframe constraints, and (2) we conducted user studies to evaluate the quality of the synthesized motion given different keyframe placement strategies: we compare our approach with a prior work~\cite{Harvey:2018:Recurrent}. Finally, we examined the effectiveness of using Motion DNA to generate motion variations.
%We trained the Global Path Prediction Network and evaluated its precision. After that, we trained the in-betweening network and evaluated its keyframe alignment precision and motion quality given sparse random keyframe inputs. We also compared its performance when given the motion transition prediction tasks defined in ~\cite{Harvey:2018:Recurrent}. Next, we examined the content and variation control effect of Motion DNA. Finally, we demonstrate two more applications of our method.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect of Range-Constrained Motion Representation}
We verify the effect of our Range-Constrained motion representation by training the same Inverse Kinematic networks as in \cite{zhou2019}. We show in Table \ref{tab:RP} that our representation and RC-FK layer outperform the other rotation representations. 
\input{table/eval_representation.tex} 

Additionally, in practice, both the ground truth training data and user's given keyframes can have bad poses, and a trained network with the RC-FK layer has the ability to correct those artifacts. For example, in Figure~\ref{fig:RC_FK_output}, left is an input frame picked from the real motion dataset where the feet are bent the wrong way. Right is our network output where the feet artifacts are fixed.

\begin{figure}
\vspace{-0.8cm}
    \includegraphics[width=0.85\linewidth]{fig/RC_FK_output.jpg}
    \vspace{-0.3cm}
    \caption{Input frame and output frame from the network with a RC\_FK layer.}
    \label{fig:RC_FK_output}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Accuracy of the Global Path Predictor}
We trained the Global Path Predictor model until it reached the precision as shown in Table \ref{tab:hip_prediction_error}. The path prediction error is 0.7 cm per frame, and only 5.5 cm after 2 seconds (128 frames) of motion. This shows that our global path prediction is quite accurate for motion prediction over a few seconds.
\input{table/eval_path_prediction.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Keyframe Alignment}
\label{sec:exp_keyframe_alignment}
We next evaluate how well our network is able to match the keyframe constraints. We first pretrain and fix the Global Path Predictor Network. We then use this to train the in-betweening network for 560,000 iterations and evaluate how well the synthesized motion aligns to the input keyframes. The input keyframes are given as the local joint coordinates plus the global root positions at some random frames. For testing, we generate 200 sets of 2048-frame-long motion sequences using random keyframes and DNA poses with the sampling scheme described in Section \ref{sec:train_details}. We calculate the mean L2 distance error of the global root joints and the local joints at the keyframes. As shown in the last two rows of Table \ref{tab:user_study_results}, the alignment error is sufficiently small that it can be easily removed by the post-processing in a way that is hardly perceptible.

We show an example rendering of the synthesized frames overlaid with the input keyframes in Figure~\ref{fig:DNA_effect}. The faint pink skeletons are the input keyframes, while the blue skeletons are synthesized by our method. It can be seen that the synthesized frames smoothly transition between the keyframes, which are specified at frame 4 and 11, and faithfully match the keyframes. More results for longer term inbetweening tasks can be found in the supplementary video.


\textbf{Dense vs. Sparse Input. }
In Section \ref{sec:input_sequence_format}, we mentioned that using a dense input format can accelerate the training. We show this effect in Figure \ref{fig:eval_sparseORdense} by evaluating the root and local joint alignment errors at the input keyframes throughout the training iterations. For each test, we generate 2048-frame-long motion sequences from 50 sets of randomly sampled keyframes and Motion DNAs, and we calculate the mean L2 errors between the input and output poses. The results show that the dense input format not only converges to lower errors but also converges much faster than the sparse input format. 
\begin{figure}
    \includegraphics[width=3.2in]{fig/eval_sparseORdense.pdf}
    \vspace{-0.2cm}
    \caption{Mean L2 errors (cm) of local joints (left) and root joint (right) at keyframes throughout the training process. Blue lines refer to the result of using the sparse input format. Red lines refer to the dense input format.}
    \label{fig:eval_sparseORdense}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparison of Different GAN Architectures}
\label{sect:comparison_gan}

\begin{figure}
    \vspace{-0.5cm}
    \includegraphics[width=\linewidth]{fig/GAN_architecture_results_comparison.jpg}
    \vspace{-0.8cm}
    \caption{Visualized synthetic and real motion data. Please see \sect{sect:comparison_gan} for an explanation of the visualization. Since all joints and a range of times are visualized in the subfigures, it is difficult to imagine the motion from this visualization, but the key takeaway is that the frequency characteristics of each joint are completely wrong for the alternative GAN approaches.}
    \label{fig:GAN_architecture_comparison}
\end{figure}

We compare the result of using different GAN architectures trained by 65,000 iterations. In Figure~\ref{fig:GAN_architecture_comparison}, each block contains three randomly picked motion sequences visualized by the coordinate values of all joints through time. From the first and second block, we can see that the real motion and our two-step GAN model's output motion have similar smooth patterns. The third block is the result of replacing the transpose convolution layers in our model with nearest neighbor upsampling layers. Although the using of upsampling layers were more popular for GAN models in the 2D image generation domain, empirically we found it leads to very noisy output and has the random mosaic patterns. The fourth block is the result of using a one-step GAN that infers both local motion and global motion simultaneously. This network diverges to bad and repeated outputs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Runtime Performance}
We conduct all our experiments on a machine with an Intel{\tiny{\textregistered}} Core$^TM$ i9-7900X CPU with 3.30GHz, 94GB memory, and a Titan Xp GPU. Our code is implemented on an Ubuntu 16.04 and uses Python 3.6 and Torch 0.4. We tested the computation time for generating motion sequences at different lengths. Table \ref{tab:speed} gives the average computation time for the network inference (forward pass) and post-processing (to enforce keyframes matching and smooth output motion), and shows that our method can achieve real-time performance for generating 15 seconds of motion. For longer motions, the system is still fast, using only within 0.4 second for generating 120 seconds of motion.

\input{table/eval_speed.tex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Motion Quality}
\label{sec:motion_quality}
We evaluated the quality of the synthesized motions from our model with a user study. We used the trained model to generate 50 34-second-long (2048 frame) motion sequences using the keyframe and DNA sampling scheme described in Section \ref{sec:train_details}. Next, we randomly and uniformly picked 100 4-second-long subsequences from these sequences. We ran an Amazon Mechanical Turk~\cite{AMT} study. We showed human workers pairs of 4-second real motions and 4-second synthetic motions, with randomization for which motion is on the left vs right. We asked the user to choose which motion looks more realistic, regardless of the content and complexity of the motion. The real motions were randomly picked from our filtered CMU Motion Capture Dataset. We distributed all of the 100 pairs in 10 Human Intelligence Tasks (HITs)\footnote{A Human Intelligence Task (HIT) is a task sent out and completed by one worker.}.  Each worker is allowed to do at most four HITs. Each HIT contains 10 testing pairs and 3 validation pairs. The validation pair contains a real motion sequence and a motion sequence with artificially large noise, so as to test if the worker is paying attention to the task. We only collected data from finished HITs that have correct answers for all three validation pairs. Ideally, if the synthetic motions have the same quality as the real motions, the workers will not be able to tell the real ones from fake ones, and the rate for picking up the synthetic ones out of all motion sequences should be close to 50\%. 

As listed in Table \ref{tab:user_study_results} under the train and test settings ``All-Random," the results show that around 40\% of our synthetic motions are preferred by the human workers, which indicates high quality. More results can be found in the supplemental video.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extension and Comparison with RTN}
\label{sect:rtn_comparison}
The related work Recurrent Transition Networks (RTN)~\cite{Harvey:2018:Recurrent} synthesizes motion transitions in a different setting than ours. Based on a fixed number of past frames and two future frames, RTN predicts a short sequence of future motion of a fixed length. Our network on the other hand supports arbitrary keyframe arrangement. In this section, we are going to examine how RTN works for short-duration motions from a single class, and how it works for long-duration motions mixed from multiple classes. We will also show the performance of our network trained under our keyframe arrangement setting, but tested under the RTN setting. 

As illustrated in the first row of Figure~\ref{fig:comparison_testSetting}, our network is designed to generate various outputs with arbitrary length and arbitrary numbers of keyframes. It is trained and tested with sparsely sampled keyframes from 79 classes of motions that contain transitions within or across classes of poses: this scenario is labelled as ``Ours-All-Random" in the experiment (Table \ref{tab:user_study_results} and Figure~\ref{fig:comparison_testSetting}). Comparatively, RTN, in the original paper, is trained to predict 1 second of walking motion. In our experiment, we also trained and tested RTN's performance for predicting 1 second of walking motions, which we illustrate in Figure~\ref{fig:comparison_testSetting} as "RTN-Walk-1s." Moreover, we tested its performance for predicting longer (4 seconds) motions trained with all 79 classes: this is labelled as "RTN-All-4s". 

Even though our model is always trained on all 79 classes of the CMU dataset (per Section~ \ref{sec:train_details}), we also test our model's generalization abilities by testing in the same scenarios as RTN. The "Ours-Walk-1s" test, as a counterpart to "RTN-Walk-1s", uses one-second motion transitions with keyframes and DNA poses all sampled from the walking class only. Likewise, the "Ours-All-4s" test, as a counterpart to "RTN-All-4s", uses four-second motion transitions with keyframes and DNA poses sampled from all classes.
%In order to perform the RTN task using the same trained model from "Ours-All-Random," we insert the same input frame pattern as RTN in the middle of a blank sequence as the input. As shown in the second and third lines, the "Ours-Walk-1s" test, as a counterpart to "RTN-Walk-1s", is set to synthesize one-second motion transitions with keyframes and DNA poses all sampled from the walking class only; the "Ours-All-4s" test, as a counterpart to "RTN-All-4s", is set to synthesize four-second motion transitions with keyframes and DNA poses sampled from all classes.

\input{table/user_study_result.tex}
\begin{figure}
    \includegraphics[width=0.9\linewidth]{fig/ComparisonRTN.pdf}
    \caption{Training and testing settings for different approaches. These are defined in \sect{sect:rtn_comparison}.}
    \label{fig:comparison_testSetting}
\end{figure}

To evaluate the quality of the synthetic motions, we generated 100 1-second sequences from "RTN-Walk-1s" and "Ours-Walk-1s," and 100 4-second sequences from "RTN-All-4s" and "Ours-All-4s" and performed the same user study on these sequences as is described in Section \ref{sec:motion_quality}. We also evaluated the keyframe alignment errors for each method based on 200 testing sequences for each method. As shown in Table \ref{tab:user_study_results}, RTN performs well in the "RTN-Walk-1s" case. However, for the 4 second case, RTN fails to generate reasonable results, with user preference rate  dropping to 2.8\% and Joint Error and Root Error increasing to 30.3 cm and 155.4 cm, respectively. On the other hand, our network, although not trained for the RTN tasks, still has reasonable user preference rate with low keyframe alignment error for both tasks. This indicates that our method not only performs well in the original training scenario but also generalizes well to new and unseen test scenarios. The user preference rates indicate that "Ours-All-4s" has higher motion quality than "Ours-All-1s." We believe this is because during training, the interval length is between 0 to 10 seconds, so the 4-second interval is closer to the expectation of the interval length during training.

\begin{figure}
    \includegraphics[width=0.8\linewidth]{fig/Variation_4_sets.jpg}
    \caption{Examples of motion variety. Within each of the four sub-figures, we visualize four poses (blue) at the same frame from a motion sequence synthesized from the same set of keyframes but with four different Motion DNAs. The pink skeletons are the target keyframe pose in the near future.}
    \label{fig:four_poses}
\end{figure}

In Figure \ref{fig:rtn_comparison_results}, we visualize qualitatively results of each method. In the first two lines, both RTN-Walk-1s model and our model is given the same past 40 frames and the future 2 frames, and they all successfully generate plausible walking transitions for the one second interval. In the last two lines, given the same input, our model generates a realistic transition while the RTN-All-4s model generates a diverging motion.


\begin{figure*}
    \includegraphics[width=\textwidth]{fig/Ours_RTN_4s_comparison.pdf}
    \caption{Examples of generating one second and four second transitions given the 40 past frames and 2 future frames. The first two rows show selected frames of a one-second transition sampled at 30 fps. The last two rows show frames of a four-second transition sampled at 60 fps. Pink skeletons visualize the input keyframes. From left to right, the blue skeletons show how the synthesized motion transitions between two keyframes. Numbers at the top-right corners are the frame indices. Corresponding results can be found in the supplementary video.}
    \label{fig:rtn_comparison_results}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Variation Control with Motion DNA}
To quantitatively evaluate the effect of our Motion DNA, we computed the two DNA errors as defined in Equation \ref{eqt:DNA1} and \ref{eqt:DNA2} of the 200 synthetic motion sequences described in Section \ref{sec:exp_keyframe_alignment}. The first DNA error is 8.4 cm, which means all of the representative poses in the motion DNA can be found somewhere in the synthesized motion sequence. The second DNA error is 6.5 cm, which means these representative poses are distributed evenly in the results. 

We also visualize the effect of Motion DNA in Figure \ref{fig:DNA_effect}. 
In the top two rows, we use motion DNA extracted from salsa poses (top row) and walking poses (second from the top) as input to the network. Under the same keyframe constraints (transparent pink skeletons), the network generates salsa (raised arms in the top row) and walking styles respectively. 
%In the first case, Motion DNA generated from salsa poses and walking poses are input respectively into the network along with the same keyframe inputs, resulting different motions with salsa and walking style. 
In the middle two rows, we use two different martial arts motion DNAs, and both results resemble martial arts but exhibit some differences in the gestures of the arms. 
A similar observation applies to the bottom two rows, where Indian Dance DNAs are used as the seed of motion. 
Figure~\ref{fig:teaser} shows another example. Under the same keyframe constraints, the synthesized two motions have different trajectories and local motions, but they both travel to the same spots at the keyframes.
Figure \ref{fig:four_poses} gives more variation examples. We show the same frame of a synthesized sequence which is generated from the same keyframes but with four different Motion DNAs. 
We observe that variations happen more frequently in the upper body than the lower body. Since the foot motion has more impact on the global movement, it is harder to find foot patterns that exactly satisfy the keyframe constraints. 

\begin{figure*}
    \includegraphics[width=0.95\textwidth]{fig/DNA_example.pdf}
    \caption{Examples of inbetweening. The pink skeletons visualize the user-specified keyframes. From left to right, the blue skeletons show how the synthesized motion transitions between two keyframes. The semi-transparent pink skeletons are the keyframes in the near future within 400 frames. Each group of two rows shows frames from two generated 2048-frame-long synthetic motion sequences given the same input keyframes but different Motion DNA. The yellow skeletons are the representative poses for the Motion DNA.}
    \label{fig:DNA_effect}
\end{figure*}



==> Long-term 3D Motion Inbetweening/introduction_new.tex <==
\section{Introduction}
%%%%%%%%Background
There is a great demand for producing convincing performances for CG characters in the game and animation industry. In order to obtain realistic motion data, production studios still rely mainly on manually keyframed body animations and professional motion capture systems~\cite{kovar2008motion}.
Traditional keyframe animations require very dense pose specifications to ensure the naturalness of the motion, which is known to be a time-consuming and expensive task, requiring highly skilled animators. 
%Motion graphs methods based on databases ~\cite{lee2002interactive, safonova2007construction,kovar2008motion} can synthesize smooth motions following user constraints by optimizing a path that combines a set of pre-captured motion clips. However, these methods are limited by the motion variations in the database and tend to perform poorly for user constraints that do not match the database motions well. Furthermore, the search space grows exponentially with the size of the dataset, which makes these approaches harder to apply on large databases. 
%Furthermore, it is nontrival to control the style of the synthesized motion.

Recent deep learning approaches have shown promising results in the automatic motion synthesis for locomotion~\cite{holden2016deep,Harvey:2018:Recurrent} and more complex performances such as playing basketball~\cite{liu2018learning} and soccer~\cite{hong2019}. However, these methods typically respect high-level controls such as the path in locomotion synthesis~\cite{holden2016deep} or task-specific goals. In contrast, when producing more expressive or complicated animations, an artist may find it useful to have more precise control on specific frames~\cite{igarashi2007spatial}. 

%%%%%%%%Problem definition
In this paper, we aim to synthesize complex human motions of arbitrary length where keyframes are given by users at flexible space-time locations with varying densities.
%in sparse and random locations with varying densities. 
%
We call this problem \emph{long-term inbetweening.} Users can iterate on their motion designs by adjusting the keyframes. 
%In this way, the users can obtain extended motion sequences by only creating a few keyframes, and can precisely adjust the frames. 
With very sparse keyframes, our system can improvise a variety of motions under the same keyframe constraints. We show one such example in~\fig{fig:teaser}. 
%In this paper, we focus on human motions.

%%%%%%%%Challenges
%e approach the long-term inbetweening problem by learning a feedforward convolutional network, which is trained on a multi-class motion capture dataset. 
%This problem is very challenging. 
%first challenge
The first question consists of how to design a network to generate realistic motions. The dataset contains a limited number of short motion clips and each clip performs only one type of motion. But in real application scenarios, one might need to simulate the transitions between keyframes from the same or different motion clips or even different motion categories, and such transitions are expensive to capture and thus do not exist in public mocap datasets. %Furthermore, it is nontrivial to generate different motions conditioned on the same keyframes and control the style of the synthesized motion. %Cynthia: The sentence above is no longer talking about the challenge of realism anymore, so I am commenting it out.

% second challenge and a bigger challenge
The second question consists of how to synthesize a sequence that can precisely follow the keyframes. To ensure the coherence of contents of the entire sequence, the motion within an interval should be synthesized holistically considering the global context of all the keyframes that could influence the current interval, instead of only two keyframes at each endpoint of the interval. Moreover, unlike previous works that generate motions based only on initial poses~\cite{li2017auto,yan2018mt}, long-term inbetweening requires the generator to perform sophisticated choreography to make sure the synthesized motion not only looks natural but also reaches keyframe poses at the specified times and positions. A small difference in the middle of a motion can result in big time or space displacements at keyframes. The reason for this is that the local movements of the limbs and the body affect the speed and direction of the character, and the integral of the velocities of sequential frames determine the global motion. Therefore, these differences can accumulate throughout the sequence and any modifications to a motion must consider both local and global effects. 

%long-term inbetweening requires a sophisticated ability to choreograph a complex sequence of motion while still managing to transit from one keyframe to the next. For example, the local limbs and trunk movements affect the speed and direction of the character, and the integral of the velocities of sequential frames determine the global motion. Therefore, a small difference in the middle of a motion can result in big time or space displacement at the end of the motion, so consequently, any modifications to a motion must consider both local and global effects.

%%%%%%%%Solution
Facing the challenges above, we propose a conditional generative adversarial network (GAN) that can learn natural motions from a motion capture database (CMU dataset)~\cite{cmu}. We propose a two-stage method, where we first synthesize local motion, and then predict global motion. Our computation is highly efficient, where one minute of motion can be generated automatically in half a second. Real-time updates are possible for shorter sequences.

To avoid synthesizing unrealistic body poses, we embed body biomechnical constraints into the network by restricting the rotation range of local joints with a Euler angle representation. Following the observations of Zhou~et~al.~\shortcite{zhou2019}, for the local joints, we carefully choose the order and the ranges of the Euler angles to avoid discontinuities in the angular representation. 
%We find that this works better than not doing so, and 
We call the integration of this angular representation with forward kinematics Range Constrained Forward Kinematics (RC-FK) layer.

We also develop a design concept called Motion DNA to enable the network to generate a variety of motions satisfying the same keyframe constraints. The motion DNA seeds are inferred from a set of reference poses which are the representative frames of real motion sequences. By choosing the type of representative frames, the user is able to influence the style of the output motion.

Here are our main contributions:
We believe that our approach is a key component for production settings where fast turn-around is critical, such as pre-visualization or the animation of secondary characters in large scenes. Furthermore, we also anticipate potential adoption of our method in non-professional content creation settings such as educational and consumer apps. 
\begin{itemize}
\item We introduce the first deep generative model that can: 1) synthesize high-fidelity and natural motions between key frames of arbitrary lengths automatically, 2) ensure exact keyframe interpolation, 3) support motion style variations in the output, and 4) mix characteristics of multiple classes of motions. Existing methods do not support all these capabilities.
\item We propose a novel GAN architecture and training approach for 
%\item To the best of our knowledge, our work provides the first solution for
automatic long-term motion inbetweening. Our two-stage approach makes the problem tractable by first predicting the local and then the global motion. 
%It is robust for different densities of keyframes and does not have sequence length limitations.
%\item As a generative model conditioned on sparse user-given keyframes, our method can generate a variety of new motion sequences from a single set of user constraints. 
\item We propose a novel Range Constrained Forward Kinematics (RC-FK) layer to embed body biomechanical constraints in the network.
\item We introduce the concept of motion DNA which allows the network to generate a variety of motion sequences from a single set of sparse user-provided keyframes.
%These motion sequences are in great demand for the game and animation industries. %cynthia: I commented the previous sentence out since I don't think we need to mention this point again especially not in the contribution summary.
\item Our method is significantly faster than state-of-the-art motion graph techniques, while providing intuitive control and ensuring high-quality output. We also plan to release our code and data to the public, upon acceptance of this paper.
%\yi{does this sentence looks fine?}
%\yi{and uses the RC-FK layer to restrict the output range of motion.} 
%In our experience, successfully training a GAN model on human motion is very hard, so our architecture and training setup is also valuable and can be a useful building block for future work. %Cynthia: I commented out the previous sentence since I am not sure we need to argue about why our contribution is a contribution here.
% To this end, we plan to release our source code and models. %(talking something about the novelty in the architecture, e.g. rotation embedding, the patch-based discriminator, the fully connected 1dCNN..., Maybe also mention that successfully training a GAN model on human motion is very hard, so the architecture design is also valuable and can be a useful reference for future works.)
%\item Maybe also add the motion IK auto-encoder for filtering the bad frames.
\end{itemize}

==> Long-term 3D Motion Inbetweening/macros.tex <==
\newcommand{\ignorethis} [1] {}

\newcommand{\sectnum    } [1] {\ref{#1}}
\newcommand{\shortsect  } [1] {\S\sectnum{#1}}
\newcommand{\sect       } [1] {Section~\sectnum{#1}}
\newcommand{\sects      } [1] {Sections~\sectnum{#1}}
\newcommand{\fignum     } [1] {\ref{#1}}
\newcommand{\fig        } [1] {Figure~\fignum{#1}}
\newcommand{\eqn        } [1] {Equation~(\ref{#1})}

%\newcommand{\colornote}[3]{} % This turns off colored notes
\newcommand{\colornote}[3]{{\color{#1}\bf{#2: #3}\normalfont}}  % This turns on colored notes

%\iftrue  % do NOT display comments
\iffalse % display comments
    % do NOT display comments
        \newcommand{\cyn}[1]{}
        \newcommand{\connelly}[1]{}
        \newcommand{\jimei}[1]{}
        \newcommand{\yi}[1]{}
\else 
    \newcommand {\cyn}[1]{\colornote{green}{Cyn}{#1}}
    \newcommand {\connelly}[1]{\colornote{blue}{Connelly}{#1}}
    \newcommand {\jimei}[1]{\colornote{cyan}{Jimei}{#1}}
    \newcommand {\yi}[1]{\colornote{red}{Yi}{#1}}
\fi

\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Imag}{Im}


==> Long-term 3D Motion Inbetweening/method.tex <==


\section{Method}

\subsection{Definitions}
In this paper, we use \emph{keyframes} to refer to user-specified root position and local pose at each joint at the specific time. We use \emph{representative frames} to refer to algorithmically extracted representative (or important) poses within a motion sequence. We use \emph{motion DNA} 
%\footnote{After deoxyribonucleic acid (DNA) in biology, which encodes genetic information.}
to refer to a random sampling of representative frames from the same motion class, embedded to a 1D hidden vector space. This \emph{motion DNA} helps characterize important properties of a motion: conditioning our network on the motion DNA allows the user to create variation in the model's output. This concept is related to the ``motion signatures" of Aristidou~et~al.~\shortcite{aristidou2018deep}. Note that our motion DNA is only roughly analogous to DNA in biology: it helps control the appearance of the overall motion but contains much less information and it is a distinct concept from the keyframes: keyframes precisely control pose at specified times. We use the following notations and a frame rate of 60 fps throughout the paper: 

\emph{Root} refers to the hip joint, which is also the root node. 

$\mathbf{S}=\{\mathbf{S}_t\}_{t=1}^N$: a sequence of synthesized skeleton poses including the global position of the root and the local position of the other joints relative to the root.

$\mathbf{S}_{t_1:t_2}$: a sub sequence of skeleton poses from frame $t_1$ to $t_2$.

$\mathbf{\hat{T}}=\{\mathbf{\hat{T}}_t\}_{t=1}^{\hat{N}}$: a set of representative frames that capture the typical characteristics of a motion class. We rotate the representative frames so that their root joints are all facing the same direction. %\yi{They all have zero root rotations.}

$N$: total number of frames.

$N'$: total number of user's keyframes.

$\phi = \{\phi_t\}_{t=1}^k$: the set of keyframe indices.

$\hat{N}$: total number of the representative frames in Motion DNA

$M$: total number of joints in the skeleton.

$\mathbf{S'}$: a joint position tensor of dimension $N \times 3M$ that contains user-specified keyframes.

$\mathbf{T}^{\mathrm{root}}_{t}$: 3D translation of the root in world coordinates at frame $t$.

$\mathbf{T}^{\mathrm{joints}}_{t}$: 3D translations of the joints relative to the root node in relative world coordinates at frame $t$. The dimension is $M \times 3$.

$\mathbf{R}^{\mathrm{root}}_{t}$: 3D rotation matrix of the root node in world coordinates.

$\mathbf{R}^{\mathrm{joints}}_{t}$: 3D rotation matrices of the joints relative to the parent joints at frame $t$. The dimension is $M \times 3 \times 3$.

%We use a frame rate of 60 fps for the whole paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \includegraphics[width=3.5in,trim={0.5in 7in 5in 0.5in},clip]{fig/overall_method_squashed.pdf}
    \caption{Method Overview. Given user-specified keyframes and the corresponding mask, we generate the local motion of every joint and every frame in a rotation representation. This is done by a fully convolutional encoder and decoder, shown in blue, which obtain extra information about style and appearance from the Motion DNA component. We then use Range-Constrainted Forward Kinematics (RC-FK) module to obtain the local joint positions. During training, a fully convolutional discriminator (shown in yellow) is used to assess realism of the produced subsequences. Finally, the local motion is passed to a global path predictor to estimate the global path of the root joint. A loss is applied to match the pose closely at the keyframes, which are indicated by black dots.}
    \label{fig:overall_method}
\end{figure}
\subsection{Method Overview}
Figure~\ref{fig:overall_method} shows our system design. 
At a high level, we use a 1-D CNN to first predict the local pose of all frames conditioning upon user-provided sparse keyframes, and then from the local pose we use another 1-D CNN to predict the global pose. We first explain the motivation of such a two-stage approach.
%We will first motivate why we used such an approach and then return to a more detailed description of the components.

%\cyn{Starting with symbol definition for method overview is very abrupt.You should talk about the overall approach at high-level terms here.}
%Given user-specified sparse keyframes, the goal of long-term inbetweening is to generate a motion sequence in which the synthesized frames match the user's input keyframes at the specified times, and also all sub-sequences of the synthesized motion look realistic. For simplicity, we use sub-sequences containing $n$ frames to measure realism.
%
%The problem could then be formulated as:
The problem of long-term inbetweening can be formulated as:
\begin{equation}
\begin{aligned}
\quad & \mathbf{S} = \mathbf{G}_0(\mathbf{S}^{'}_{\phi})\\
\quad & \min_{\mathbf{G}_0}{ \sum_{t=1}^{N-n} {\mathcal{L}_\mathrm{realism}(\mathbf{S}_{t:t+n})}}\\
\quad & \mathrm{s.t.} \forall t\in \phi, \mathbf{S}_{t} = \mathbf{S}^{'}_{t}    \\
%\quad & \mathbf{S} = \mathbf{G}(\mathbf{S}^{'}_{\phi})\\
%\quad & \max_{\mathbf{G}}{ \sum_{t=1}^{N-n} {P(\mathrm{real} | \mathbf{S}_{t:t+n})} - \sum_{t\in \phi} {\|\mathbf{S}_{t} - \mathbf{S}^{'}_{t}\|^2}} \\
%\textrm{s.t.} \quad & \mathbf{S}_{\phi_j}=\mathbf{S}^{'}_{\phi_j},  \textrm{for } \phi_j\in \{\phi_1,...\phi_k\}\\
\end{aligned}
\end{equation}
%Connelly: removed all this unnecessary info since we should have already defined it previously
%where $\mathbf{S}=\{\mathbf{T}^{root}_{t}, \mathbf{T}^{joints}_{t}\}_{t=1}^{N}$ is the synthesized motion sequence that contains global translations of the root joint $\mathbf{T}^{root}_{t}$ and local translations of the other joints $\mathbf{T}^{joints}_{t}$, and $\mathbf{S}^{'}_{\phi}=\{\mathbf{T}'^{root}_{\phi}, \mathbf{T}'^{joints}_{\phi}\}$ is the pose at keyframes $\phi = \{\phi_1,...\phi_k\}$. 
where $\mathbf{S}$ is the synthesized motion sequence that contains all joint information, $\mathbf{S}^{'}$ is the user-specified pose, which is defined for the keyframes at times $\phi$, $\mathbf{G}_0$ is a generative model, and $\mathcal{L}_\mathrm{realism}$ is some loss that encourages realism. For simplicity, we use sub-sequences containing $n$ frames to measure realism. 
%
Note that given very sparse keyframes, there might be multiple good solutions. %Unfortunately, we are not aware of any simple metrics that can measure the realism of the generated motions, and we are also not aware of any previously published generative functions $\mathbf{G}$ that can create complex motions based on only a few keyframes. % Connelly: removed previous sentence. There does not seem to be any point and it restated what was already said in the intro.

One approach to measure realism is to use a generative adversarial network (GAN). A GAN could be conditioned on the user-specified keyframes $\mathbf{S}^{'}$, uses a discriminator to measure the realism, and uses a generator to hallucinate complex motion while simultaneously matching the keyframes and deceiving the discriminator. 
%
However, we found that empirically, training a GAN to generate global and local motions together is much more unstable than training it to generate local motions only. This is partially because the output realism is very sensitive to global motion, e.g. 10 degree tilt on root while walking leads to impossible motion, but the local poses are still good. Predicting local motions alone significantly simplifies the problem and allows the network to focus on generating realistic local poses.
%With limited amount of training data, the training is more stable if the generator hallucinate local motions first.  
%We will provide a more detailed explanation for why this happens and corresponding experimental results in Section~\ref{}. 
Fortunately, we found that the global motion can be inferred from the synthesized local motions using a pre-trained and fixed network that we call the ``global path predictor". 
% Connelly: removed confusing sentence below, replacing it with something more intuitive.
% Fortunately, we found that the trajectory of the root can be inferred from the synthesized local motions and the initial position of the root and we can optimize for a function $\mathbf{\Upsilon}$, such that $\mathbf{T}^{root} = \mathbf{\Upsilon}(\mathbf{T}^{joints}, \mathbf{T}^{root}_{0})$. 
%
%cynthia: the setence below is repetitive.
%Although the generator doesn't explicitly output the global path, the global path is implicitly hidden in the sequence of the output local motion sequence. 
%
Thus, we design a two-stage method to first generate the local motions and then the global path. We reformulate the optimization as:
\begin{equation}
\begin{aligned}
\quad & \mathbf{T}^{\mathrm{joints}} = \mathbf{G}(\mathbf{S}^{'}_{\phi}),  \mathbf{T}^{\mathrm{root}} = \mathbf{\Upsilon}(\mathbf{T}^{\mathrm{joints}})\\%, \mathbf{T'^c})\\ % Connelly: removed T'^c it is confusing
\quad & \mathbf{S}_{t} = \{\mathbf{T}^{\mathrm{root}}_{t}, \mathbf{T}^{\mathrm{joints}}_{t}\}\\
\quad & \min_{\mathbf{\Upsilon}, \mathbf{G}} \sum_{t=1}^{N-n} {\mathcal{L}_\mathrm{realism}\left( \mathbf{T}^{\mathrm{joints}}_{t:t+n}\right)} + \gamma \sum_{t\in \phi} {\|\mathbf{S}_{t} - \mathbf{S}^{'}_{t}\|^2}\\
%\textrm{s.t.} \quad & T^{root}_{\phi_j}=T'^{root}_{\phi_j}, T^{joints}_{\phi_j}=T'^{joints}_{\phi_j},  \textrm{for } \phi_j\in \{\phi_1,...\phi_k\}\\
\end{aligned}
\end{equation}

%Here there are two networks. 
The first network $\mathbf{G}$ is a generator network that is conditioned on keyframes and outputs the local motion $\mathbf{T}^{\mathrm{joints}}_t$. The second network $\mathbf{Y}$ is a global path predictor, which is conditioned on the local motion and predicts the global motion, that is the velocities $\mathbf{dT}^{root}_t = \mathbf{T}^{root}_{t+1} - \mathbf{T}^{root}_t$, which can be summed to recover the global motion $\mathbf{T}^{root}_t$. Because the global path predictor is conditioned on the local motion, and the local motion is conditioned on the keyframes, this means the global path predictor indirectly receives information related to the keyframes. We can also view the split into local and global motion as being related to learning disentangled representations (e.g. ~\cite{gonzalez2018image}): by forcing one network to generate only local pose and the other network to integrate up these poses into global motion, we simplify the problem into two coupled, but more specialized learning tasks. For $\mathcal{L}_\mathrm{realism}$, we use a GAN loss (\sect{sec:generator_and_discriminator}). Finally, we use an $L^2$ loss to measure the mismatch between the generated frame $\mathbf{S}_{t}$ and the user's keyframe $\mathbf{S}^{'}_{t}$. 
%The hyperparameter $\gamma$ controls the loss weight. 
%We can optionally postprocess the generated motion to guarantee that the keyframes are matched exactly (\sect{sec:post}). 
In practice, we first train the global path predictor $Y$ using the motions in the CMU motion dataset~\cite{cmu}. After pretraining the global path predictor, we then freeze its weights and train the generator $\mathbf{G}$. 
%\cyn{what is $\epsilon$? should it be $\Upsilon$?}
%Note that the temporal locations of given keyframes in the input sequence specify timing constraints at a fixed temporal resolution, 60 fps.
%The above sentence is already mentioned earlier under section 3.1.

Most deep learning based motion synthesis works~\cite{Harvey:2018:Recurrent, MordatchLAPT15, villegas2018neural} use recurrent neural network (RNN) which is specifically designed for modeling the dynamic temporal behavior of sequential data such as motion. However, traditional RNN only uses the past frames to predict future frames. 
Harvey and Pal~\shortcite{Harvey:2018:Recurrent} proposed Recurrent Transition Network (RTN), a modified version of LSTM, which generates fixed-length transitions based on a few frames in the past and a target frame in the future. However, RTN cannot process multiple future keyframes spaced out in time and is therefore only suitable for modeling simple locomotion which does not need to take into account a global context specified by multiple keyframes. 
%A solution for RNN to foresee the future is to feed thearget future frames into the current state as designed by Harvey and Pal~\shortcite{Harvey:2018:Recurrent} which can generate smooth transition in a fixed time interval, but it is still an inflexible structure for the need of seeing multiple future poses in different time intervals. 
In contrast, a 1-D convolutional network structure that performs convolutions along the time axis is more suitable for our scenario, because multiple keyframes can influence the calculation of a transition frame given large enough network receptive field. 
%it can perceive all the user's keyframes in a window size determined by its biggest receptive field. %Thus, the encoder, decoder and discriminator in our method are all built with fully convolutional layers and can process arbitrary length of motion (not really true, the length must be the multiple of 64). 
Thus, we use 1-D convolutional neural network for our global path predictor, motion generator and discriminator. 

%We now discuss the different components of our system illustrated in Figure~\ref{fig:overall_method}. 
As illustrated in Figure~\ref{fig:overall_method}, given the global coordinates of the root and the local positions of other joints at keyframes (black dots and frames in the leftmost region), a generator synthesizes the local pose in rotation representation for all the frames. A motion DNA vector is additionally fed into the generator to enable varied outputs and encourage the output to match in style. Next, a Range-Constrained Forward Kinematics (RC-FK) layer translates the local pose in rotation representation to 3D positions, which are then fed into the global path predictor to generate the trajectory of the root. We developed the RC-FK layer to remove discontinuities in the angle representation, which can harm learning~\cite{zhou2019}. The remaining sections will discuss each of the components in details.
%Input with both the given local poses and global root coordinates, a generator followed by a novel Range-Constrained Forward Kinematics Layer (RC-FK) outputs the whole sequence of local poses which are then fed into the Global-Path-Predictor to synthesize the whole path. 
%For the generated local motion, we use a discriminator to check the realism of each sub-sequence. We also apply an $L^2$ reconstruction loss at keyframes for both the local poses as well as the global root coordinates. 
%Cynthia: The previous sentence is mentioned earlier in the section.
%Both networks are fully convolutional and thus, able to process arbitrary length of motion sequences. 
%Cynthia: The previous sentence seems a bit out of place

%In the following sections, we start by explaining the two motion representations we use in our method and the RC-FK layers designed for simultaneously restricting the range of motion according to human body flexibility and ensuring the continuity in the representation (Section~\ref{sec:RC_FK}). Then we explain the architecture for the global path predictor (Section~\ref{sec:global}).  Next, we explain how we design the input format, the local motion generator, the discriminator and the Motion DNA with the corresponding loss functions (Section~\ref{sec:generation}).
%Next, we explain how to sample training instances and encourage the network to generate variations given the same input keyframes (Section~\ref{sec:variations}). 
%Finally, we introduce an optional post-processing method to exactly enforce keyframe constraints (Section~\ref{sec:post}) and discuss remaining training details (Section~\ref{sec:train_details}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Range-Constrained Motion Representation}
\label{sec:RC_FK}
As a reminder, throughout our network, following Zhou~et~al.~\shortcite{zhou2019}, we would like to use continuous rotation representations in order to make the learning process converge better. A skeleton's local pose at a single frame can either be defined by the local joint translations $\mathbf{T}^{\mathrm{joints}} = \{\mathbf{T}_i\}_{i=1}^M$ or hierarchically by the relative rotation of each joint from the parent joint $\mathbf{R}^{\mathrm{joints}} = \{\mathbf{R}_i\}_{i=1}^M$. By denoting the initial pose as $\mathbf{T}^{\mathrm{joints}}_{0}$ (usually a T pose) and the parent index vector $\varphi_{\mathrm{child}\_\mathrm{id}}=\mathrm{parent}\_\mathrm{id}$, we can map the rotation representation to the translation representation by a differentiable Forward Kinematics function $FK(\mathbf{R}^{\mathrm{joints}}, \mathbf{T}^{\mathrm{joints}}_{0}, \varphi)= \mathbf{T}^{\mathrm{joints}}$ ~\cite{villegas2018neural}.

%Cynthia: I don't quite understand the sentences below and why they are mentioned here. I am commenting them out for now.
%Due to the flexibility limitation of human body, the mapping is one-to-one and both the translation and rotation representations are continuous along the time axis for a normal human body. However, without the restriction on the rotation range, the mapping from the former one to the latter one is not unique. 
%
Many public motion datasets do not capture the joint rotations directly, but instead use markers mounted on human performers to capture the joint coordinates, which are then transformed to rotations. Due to insufficient number of markers, the imprecision of the capture system, and data noise, it is not always guaranteed that the calculated rotations are continuous in time or within the range of joint flexibility. %\yi{If time permits, insert a figure here showing a bad pose.}. 
%Cynthia: I feel like the paper is getting pretty long. The sentence below might not be necessary
%For example, suppose we put a marker on the wrist and another one on the hand, the coordinate of the wrist and the marker on the hand won't change with either palm up or palm down, while the rotation of the wrist changes 180\degree. 
In contrast, joint positional representation is guaranteed to be continuous and thus are suitable for deep neural network training~\cite{zhou2019}. Therefore, we use the joint translations as the input to our generator and discriminator. However, for the motion synthesized by the generator network, we prefer to use a rotation representation, since we want to guarantee the invariance of the bone length and restrict the joint rotation ranges according to the flexibility of the human body. These kinds of hard constraints would be more difficult to enforce for a joint positional representation.% Then the question is how to restrict the range of the generated join rotations.
%\^{T}

% Connelly: removed Fig 3 because it is confusing.
% \begin{figure}
%     \includegraphics[width=3.2in]{fig/IK_world_vs_joint}
%     \caption{Example of local joint rotation coordinates. Left column shows the local coordinate systems that are aligned with the world coordinate at the initial state. Right column shows using the local coordinate systems in the joint coordinates. The first line shows the initial state, the second line shows that the first joint (left) rotates counterclockwise by 20 degree, and the third line shows the second joint (right) then rotates counterclockwise by 30 degree. The coordinates with solid lines are the original ones and the coordinates with dash lines are the updated ones.
%     Link for editing:\href{https://docs.google.com/drawings/d/1zFFB2BaLl2Tum-XiUckGwjUvvrSBkktFAO9bq7r9J38/edit?usp=sharing}{click me}}
%     \label{fig:IK_world_vs_joint}
% \end{figure}

%\cyn{I don't think Figure~\ref{fig:IK_world_vs_joint} is necessary}
We now explain the rotation representation we use for the local joints. We define a different local Euler angle coordinate system for each joint with the origin at the joint, x and y axis perpendicular to the bone and the z axis aligned with the child bone (and if a joint has multiple child bones, then the mean of the child bones). %as shown in the right column in Figure~\ref{fig:IK_world_vs_joint}, then
% Connelly: removed ref to Fig 3 above
%We use the Tait-Bryan Euler angles convention, where the order of rotation is referred to as x-z'-y'' for intrinsic rotations or y-z-x for  extrinsic rotations~\cite{wiki:euler_angles}.
Due to joint restrictions on range of motion, the rotation angles around each axis should fall in a range, $[\alpha, \beta]$, where $\alpha$ is the minimal angle and $\beta$ is the maximal angle. We have the neural network output the Euler angles $v=(v_x, v_y, v_z)^T\in \mathbb{R}^3$ for each joint except for the root joint and then map them to the feasible range by: 
\begin{equation}
u = \left[\begin{array}{c}
u_x \\
u_y \\
u_z \\
\end{array}
\right]
=
\left[\begin{array}{c}
(\alpha_x-\beta_x)\tanh(v_x)+(\alpha_x-\beta_x)/2 \\
(\alpha_y-\beta_y)\tanh(v_y)+(\alpha_y-\beta_y)/2 \\
(\alpha_z-\beta_z)\tanh(v_z)+(\alpha_z-\beta_z)/2 \\
\end{array}
\right]
\end{equation}
We can move from the relative rotation of the joints to world coordinates in the usual way for forward kinematics by composing the relevant 4x4 homogeneous rotations and translation matrices.
%The local rotation matrix $R^l_l$ in the local coordinate system can be computed by multiplying the rotation matrices derived from the rotation angles along each of the three axes. The local rotation matrix $R^w_l$ in the world coordinate system (also centered at the joint) can be computed as $R^w_l = M^{
%{lw}} R^l_l M^{wl}$, where $M^{lw}$
%is the transformation matrix from the local coordinate system to the world coordinate system and $M^{wl}$ from world to local. All of these matrices are expressed in 4x4 homogeneous coordinates.

%\cyn{How do you calculate $M^{lw}$ and $M^{wl}$?}
%\cyn{Mention how did you obtain the range at each joint? Provide all the range values in appendix or supp?}
%\yi{Will add them later}

Although it is convenient to enforce the rotation range constraint, the Euler angle representation can have a discontinuity problem, which can make it hard for neural networks to learn~\cite{zhou2019}. 
%So far we are able to restrict the output joint rotations in a feasible range, however, we still have not solve the singularity problem in such a Euler angles representation. As pointed by (our rotation paper), the Euler angle representation have discontinuity problems that make it hard to be approximated perfectly by neural networks. 
The discontinuity happens when the second rotation angle reaches $(-90\degree$ or $ 90\degree)$, which is known as the Gimbal lock problem. 
%Training network using Euler angles without carefully handling this singularity will result in unavoidable big errors at certain rotations. 
Fortunately, each body joint except the hip joint has at least one rotation axis along which the feasible rotation range is smaller than $(-90\degree, 90\degree)$. Thus, we can avoid Gimbal lock by choosing the order of rotations accordingly. 
%of the multiplication of the three rotations for each joint. 
Therefore, we compute the rotation matrix of the left and the right forearms in the $Y_1X_2Z_3$ order and the other joints in the $X_1Z_2Y_3$ order as defined by Wikipedia for the intrinsic rotation representation of Tait-Bryan Euler angles~\cite{wiki:euler_angles}. For the hip, since there is no restriction in its rotation range, to avoid discontinuities, we use the continuous 6D rotation representation defined in~\cite{zhou2019}.

The detailed information regarding the range and order of the rotations at each joint can be found in the appendix.

%\cyn{Comment this out if we don't have time for the appendix.}
%The details of the functions for mapping the neural network outputs ${v_1, v_2,.., v_N}$ to local joint rotation matrices $s_{rot}$ and finally to the joint positions $s_{pos}$ can be found in the code in the appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Global Path Predictor}
\label{sec:global}
We infer the global translations of the root using a 1D fully convolutional network which takes the synthesized local joint translations as input and outputs the velocity sequence of the root joint $\mathbf{dT}^{root}_t = \mathbf{T}^{root}_{t+1} - \mathbf{T}^{root}_t$. The architecture is in Table \ref{tab:network_architectures} of the appendix. The network is trained with the ground truth motions in CMU Motion Capture dataset~\cite{cmu}. 
%The global translation of the root is infered by a pre-trained global path predictor (GPP). 
%we use the real motion datset to supervise the training of GPP. 
%GPP is also a fully convolutional network that can handle arbitrary length of sequence. 
%The input of the network is a sequence of local joint translations $\mathbf{S}^{T_{joints}}$ which is the output of the RC-FK module.
%The output is the sequence of velocity $\mathbf{S}^{dT^{root}}$. $\mathbf{dT}^{root}_t = \mathbf{T}^{root}_{t+1} - \mathbf{T}^{root}_t$
Between any two times $t_0$ and $t$, we can compute the displacement in the root position as:
\begin{equation}
    \mathbf{\Delta}^{root}_{t_0->t} = \sum_{i=t_0}^{t}\mathbf{dT}^{root}_i
\end{equation}


To prevent drifting due to error accumulation in the predicted velocity, we penalize root displacement error in each $n$-frame interval, $n=1,2,4,...,128$.
\begin{equation}
    L = \frac{1}{8} \sum_{q=0}^{7} \frac{1}{N-n}\sum_{t=1}^{N-n} ||\mathbf{\Delta}^{root}_{t->t+n} - \mathbf{\Delta}'^{root}_{t->t+n}||^2
\end{equation}
where by abuse of notation, $n=2^q$, $\mathbf{\Delta}^{root}_{t->t+n}$ is the root displacement from frame $t$ to frame $t+n$ calculated using the predicted $\mathbf{dT_{t+1,..., t+n}}$ and $\mathbf{\Delta'}^{root}_{t->t+n}$ is the corresponding ground truth displacement, that is, the difference between the ground truth frames.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Local Motion Generation}
\label{sec:generation}
\begin{figure}
    \includegraphics[width=3.3in,trim={0 1cm 0 0},clip]{fig/local_GAN}
    \caption{Network Architecture for Local Motion Generation. As explained in Section~\ref{sec:RC_FK}, $\mathbf{V}_t$ contains a 6-D vector that represents the rotation of the root and (M-1) 3-D vectors that represent the rotation of the other joints. $\mathbf{R}_t$ contain the 3x3 rotation matrices for all the joints. $\mathbf{T}_t$ and $\mathbf{\hat{T}}_t$ contain the local translation vectors for all the joints except for the root joint. 
$\mathbf{w}$ is concatenated with each $\mathbf{z}_t$ to be fed into the decoder.}
    \label{fig:local_GAN}
\end{figure}


The local motion generation module takes as input a sequence of vectors that capture the locations and values of the keyframes and outputs the local motion for the whole sequence. 
As shown in Figure \ref{fig:local_GAN}, it is composed of five parts: 
(1) an encoder to encode the input sequence into a sequence of 1-D latent vectors $\mathbf{z}_t \in \mathbb{R}^{1024}$, 
(2) a Motion DNA encoder to encode a set of randomly picked representative frames $\mathbf{\hat{T}}$ into a 1-D latent vector $\mathbf{w}\in \mathbb{R}^{1024}$, 
(3) a decoder to synthesize the local motion of the entire sequence in the rotation representation, 
%$\mathbf{S}^V$, 
(4) a Range-Constrained Forward Kinematic (RC-FK) module to transform the local motion from the rotation representation back to the positional representation $\mathbf{S}$, and
(5) a discriminator to encourage realism of the generated sub-sequences. %All of these except for the RC-FK module are neural networks: the motion DNA network is a multilayer perceptron, and the rest are fully convolutional.

In the following subsections, we first explain our dense keyframe input format, then we discuss the architecture of our generator and discriminator, and the losses we use at training time. We then explain how our Motion DNA works.

%The format of $\mathbf{I}_t$ will be explained in Section \ref{sec:input_sequence_format}. 


\paragraph{Dense Keyframe Input Format.}
\label{sec:input_sequence_format}
The local motion generator receives sparse input keyframes that are specified by the user. We could format these keyframes in either a sparse or dense format: we will explain the sparse format first, because it is easier to explain, but in our experiments, we prefer the dense format, because it accelerates convergence. In the case of the \emph{sparse input format}, the inputs are: (1) a mask of dimension $N \times 3M$ that indicates at each frame and each joint, whether the joint's coordinate values have been specified by the user, and 
%(1) a sequence of $M \times 3$ dimensional masks that indicates whether the three coordinate values (xyz) of each joint are given by the user, and 
(2) a joint position tensor $\mathbf{S'}$ of dimension $N \times 3M$ that contains user-specified world-space joint positions at keyframes $\phi$ and zero for the rest of the frames. These are shown in the second and third rows in Figure~\ref{fig:input_format}. This sparse input format can encode the pose and timing information of the users' keyframes and is flexible for cases of partial pose input, e.g. the user can give the root translation without specifying the local poses. However, since the keyframes are sparse, the input sequence usually contains mostly zeros, which results in useless computation in the encoder. Thus, we prefer the \emph{dense input format}, which is shown in the fourth and fifth rows of Figure~\ref{fig:input_format}. In the dense input format, each frame in $\mathbf{S'}$ gets a copy of the pose from its closest keyframe. 
The mask is also replaced with a distance transform, so the values at the keyframes are zero, and the values at the other frames reflect the absolute difference in index between that frame and a closest keyframe. 
%The values in the masks are also propagated to the whole sequence noted as $\mathbf{DM}$ in the way that $\mathbf{DM}_{t} = \phi_i - t$, $\phi_i$ is the closest keyframe index to frame $t$. 
The dense input format increases the effective receptive field of the generator, since with keyframes duplicated at multiple input locations, each neuron in the bottleneck layer can see a larger number of keyframes. Empirically, this representation also leads to a faster network convergence. 

%Using the dense input format, the maximum window size of the generator for perceiving the input keyframes are nearly doubled to 636 frames, and we also empirically find that the convergence of the network becomes faster (refer to the experiment section if I have time to put it in). 

\begin{figure}
    \includegraphics[width=3.3in]{fig/input_format.png}
    \caption{Input Format for Local Motion Generator. The first row contains the frame indices. The second and third rows show the sparse input format, and the fourth and fifth rows show the dense input format. 1s and 0s in the second row indicate the presence and absence of keyframes. $S'_{\phi}, \phi=3, 64, 67$ are the poses at user-specified keyframes.
    }
    \label{fig:input_format}
\end{figure}


\paragraph{Generator and Discriminator Architecture.}
\label{sec:generator_and_discriminator}
The encoder contains six convolutional layers that reduce the input dimension by $2^6$ = 64 times, and the decoder contains eight convolutional layers and six transpose convolutional layers to upsample the latent representation to the original input dimension. The size of the receptive field at the bottleneck layer is 318 (5.3 seconds) frames. With the dense input format introduced in Section~\ref{sec:input_sequence_format}, the effective receptive field becomes 636 frames (10.6 seconds): this is theoretically the longest  time interval between any neighbouring keyframes, because otherwise the synthesized transition at a particular frame will not be dependent on the two adjacent keyframes. 
%that the network can potentially guarantee to synthesize natural transitions because beyond this interval, the network cannot see the two neighboring keyframes. 
%In Section~\ref{sec:input_sequence_format}, we provide a method to double the size of the receptive field. 

The discriminator takes as input the entire synthesized sequence, passes it to seven convolutonal layers (6 layers perform downsampling and 1 layer maintains the input dimension) and outputs $N/64$ scalars $y_t$. The discriminator looks at all the overlapping sub-sequences ($N/64$ sub-sequences of length 64 frames each) and predicts whether each of them looks natural (one output scalar per sub-sequence). The receptive field of the discriminator is 190 frames: this is the length of the sub-sequence that each $y_t$ is responsible for. 
%Cynthia: I feel like the detail below is not necessary to mention here.
%We add paddings to each layer carefully so that contributions of the frames at the two ends of the whole sequence will be the same as the ones in the middle \yi{I can add one figure to explain this if people find it confusing}. 

%\cyn{Talk a little bit about the intuition here? Why they help with mode collapse? The residual layer is unconventional, should probably talk about intuition too. Conventional one does not have $\sigma$. In the ideal case, it will be great to have ablation study to show how much difference these complicated design make.}
During experiments, we found that generators using vanilla convolutional layers cannot precisely reconstruct the input keyframes and tend to to have mode collapse, by synthesizing similar motions for different inputs. We hypothesize that this is because the network is too deep and the bottleneck is too narrow. To this end, we introduce a modified residual convolution layer and a batch regularization scheme:
%The following is the equation of the residual block on the simple condition with unchanged input and output channel size and sequence length.

\begin{equation}
\begin{aligned}
\quad & \mathbf{x}'=\text{conv}(\mathbf{x})\\
\quad & \text{residual}(\mathbf{x}) =\text{PReLU}(\text{affine}(\mathbf{x}')) + \sqrt{1-\sigma}\mathbf{x} \\
\quad & \mathbf{y}=\sqrt{\sigma}\text{residual}(\mathbf{x}) + \sqrt{1-\sigma}\mathbf{x} \\
\end{aligned}
\label{eqn:our_residual_convolution}
\end{equation}

Here $\mathbf{x}$ is the input tensor and $\mathbf{y}$ is the output. PReLU() is an activation function called Parametric Rectified Linear Unit~\cite{He:2015}. affine() is a learned affine transformation, which multiplies each feature elementwise by a learned scale-factor and adds to each feature elementwise a learned per-feature bias. conv() stands for the convolutional filter with learnable kernels. The residual ratio $\sigma$ is a scalar from 0 to 1. 
%\jimei{Is there a reference for this residual network design?}\cyn{Is equation 6 our own contribution? Can we talk more about the intuition here and how do we justify this modified residual layer?}\yi{I added the following intuition which is potentially nonsense.} 
In our network design as shown in the appendix, we set $\sigma$ in a decreasing manner. The intuition here is that the layers closer to the output mainly add low-level details, and therefore we want to pass more information directly from the previous layer, especially near keyframes. 
%A batch regularization loss term is applied on $x'$ during training.

\paragraph{Losses for GAN and Regularization.}
%The detailed implementation of the residual blocks for transpose CNN and for changed input and output channel size and sequence length can be found in our future released code. 

We applied the Least Square GAN Losses~\cite{Mao2017LeastSG} on our generator and discriminator. %The discriminator learns to distinguish real motion sequences from generated ones 
We use 1 as the real label and -1 as the fake label and therefore $y_t^{real}$ should be close to 1 and $y_t^{fake}$ should be close to -1. 
%We design the loss functions that force the discriminator to output $y_t$ to be close to $1$ for a real motion sequence and $-1$ for a fake motion sequence as
\begin{equation}
\begin{aligned}
%\quad & L^D_{real} = 1/(N/64)\sum_{t=1}^{N/64}{(y_t^{real}-1)^2} \\
%\quad & L^D_{fake} =  1/(N/64)\sum_{t=1}^{N/64}{(y_t^{fake}+1)^2}
\quad & L^D = 1/(N/64) (\sum_{t=1}^{N/64}{(y_t^{real}-1)^2} + \sum_{t=1}^{N/64}{(y_t^{fake}+1)^2})
\end{aligned}
\end{equation}

For the generator, we want the corresponding $y_t$ to be close to neither -1 nor 1. According to the Least Square GAN paper~\cite{Mao2017LeastSG}, one can use any value in [0, 1), and based on experiments, we chose 0.2361, so we have:
\begin{equation}
\begin{aligned}
L^G_{adv} = 1/(N/64)\sum_{t=1}^{N/64}{(y_t^{fake}-0.2361)^2} 
\end{aligned}
\end{equation}

Before we feed synthesized local motion sequences $\mathbf{S}$ into the discriminator, we replace the pose at the keyframe locations with the input pose, because we found that this encourages the network to generate smooth movement around the keyframes. 

For our problem, we found that standard batch normalization~\cite{ioffe2015batch} does not work as well as a custom batch regularization loss. This appears to be because when using batch normalization, different mini-batches can be normalized differently due to different mean and standard deviations, and there may also be some difference between these values between training and test times. We apply the following batch regularization loss to each modified residual convolution layer in the generator and discriminator:
\begin{equation}
    L_{\mathrm{br}} = 1/D \sum_{\mathbf{x}\in\{\mathbf{X}'\}} (||\mathrm{E}(\mathbf{x}')||^2_2 + ||\log(\sigma(\mathbf{x}'))||^2_2)
\end{equation}
Here $\{\mathbf{X}'\}$ is the set of outputs of the convolution layers in the residual block, D is the total dimension of $\{\mathbf{X}'\}$, $\mathrm{E}$ and $\sigma$ refer to the sample mean and standard deviation of the features. We also found empirically that this loss helps encourage the diversity of the output motions and avoid mode collapse.% For our problem, we found that this soft regularization is more robust than batch normalization, because it avoids the problem where different mini-batches can be normalized differently due to different mean and standard deviations, and there may also be some bias between these values at training and test times. 
%\cyn{give out the exact network architecture especially if we claim the architecture design as novelty. Also need to talk about intuition why the new architecture is better than previous ones.}\yi{The following sentence is all I can add.} 


\paragraph{Losses for Keyframe Alignment.}
%Cynthia: I think the setence below is already mentioned somewhere in the begining
%After pretraining the global root motion predictor, we fix its weights and plug it into the end of our local motion generator, then we start to train the whole network for synthesizing the global and local motion.
%
To further enforce the keyframe constraints, we use L2 reconstruction loss on the position vectors of all non-root joints at keyframes. 
%we use the following reconstruction loss on the local motions at the keyframes,
%Cynthia: I feel like the reconstruction loss is very easy to understand and does not need an explicit equation here
%\begin{equation}
% L^G_{key} =  1/N'\sum_{i=1}^{N'}{
% ||\mathbf{T}^{joints}_{\phi_i}-\mathbf{T}'^{joints}_{\phi_i}||^2_2} 
%\end{equation}

However, for the root (hip) node, applying such a naive L2 distance calculation is problematic. We show one example of why this is the case in Figure~\ref{fig:root_distance}. In that example, the output root trajectory matches well the input in terms of direction, but a large error is reported because the synthesized and target point clouds are not well-aligned, due to a cumulative drift in prediction over time. 
%A vanilla loss function of the root translation for training the whole network can be 
%\begin{equation}
%    L_{root} = \frac{1}{N'}\sum_{t\in\{\phi\}}||(\mathbf{T}^{root}_{t}-\mathbf{T}^{root}_{t0})-(\mathbf{T'}^{root}_{t}-\mathbf{T'}^{root}_{t0})||^2_2
%\end{equation}
%But this formula is not ideal because in cases like in the left part of Figure \ref{fig:root_distance}, the output root path matches the input key root sequence in terms of direction, but with the big displacement, loss can still be big. 
To fix this, we recenter the output path by placing the mean of the output root trajectory $\mathbf{T^c}$ at the mean of the input root trajectory $\mathbf{T'^c}$, where both means are taken only over keyframes. This is shown in the right part of Figure~\ref{fig:root_distance}. The updated loss function becomes:
\begin{equation}
    L_{root} = \frac{1}{N'}\sum_{t\in\{\phi\}}||(\mathbf{T}^{root}_{t}-\mathbf{T^c})
    -(\mathbf{T'}^{root}_{t} - \mathbf{T'^c})||^2_2
\end{equation}

This is equivalent to performing a least-squares fit over all translations. Least-squares fits over all rigid transforms have also been studied~\cite{arun1987least,lorusso1995comparison}. We opted to not fit the rotational components because such a rotation would induce changes in the orientation for the local motion, which could make the local motion harder to learn, since the target orientation would not match the input keyframes and would depend upon this downstream normalization. 

\begin{figure}
 \includegraphics[width=0.7\linewidth]{fig/root_l2_error.png}
    \caption{Root translation error calculation. The blue path is the synthesized root path, and blue dots are the synthetic root positions at the keyframes. Red crosses indicate the input root positions at the keyframes. %\cyn{I actually don't quite understand the figure here. Why does the left case happen if you don't do recentering? It does not align with the text description in section 3.5. Yi, can you please double check? The blue path and the red dot do not have the same direction.}
    %and dash lines indicate the displacement between the synthesized roots and input keyframe roots
}
    \label{fig:root_distance}
\end{figure}

\subsubsection{Motion DNA}
To encourage the network to hallucinate different motion sequences following the same keyframe constraints, we introduce a novel conditioning method that we call Motion DNA. By changing the Motion DNA, users can provide some hints about the type of motion to be generated. 
%While generating natural motions that strictly follow the input sparse keyframes, we also designed a scheme called Motion DNA to encourage the network to hallucinate different motions under the same keyframe constraints. With Motion DNA, the users are even allowed to give weak control on the type of the output motion.

We were motivated to create such a scheme because we noticed that motion within the same class can sometimes exhibit dramatically different styles and it is impossible to classify all types of motions by limited labels.  For example, in the CMU Motion Capture dataset, a class called ``animal behaviors" contains human imitations of different animals such as elephants and monkeys, but their motions don't share any common features.

% Connelly: I found the below paragraph confusing and I don't agree about the representation about static classes. So I simplified it to the above one. 
%The question is how to encode the motion type and how to condition the network to generate the desired type of motion. 
%Motion, as dynamic signals, cannot be adequately represented by a fixed-length static code. It is also hard to reliably classify motion into predefined discrete classes. Sometimes, motion within the same class can exhibit dramatically different styles. For example, in the CMU Motion Capture dataset, a class called "animal behaviors`` contains human imitations of different animals such as elephants and monkeys. These motion sequences though belong to the same class, do not have enough similarities in feature space. Thus, it's hard to use a static code to represent the wide range of motion variations per class. 

Instead of using labels, we found that a small set of representative frames of a motion sequence contain discriminative and consistent features that can well represent the characteristics of a particular type of motion. For example, the yellow skeletons in the fifth line in Figure \ref{fig:DNA_effect} are the representative frames extracted from a motion sequence, and it is not hard to tell that they are extracted from a martial arts sequence. We identify representative frames as those that have the maximum joint rotation changes from their adjacent frames. The extracted representative frames can be injected into the generator to control the characteristics of the generated motion. The advantage of using the representative frames as the controlling seeds is that it can be applied to general types of motions and the user can explicitly define their own combination of the representative frames.


To encode the set of representative frames into a Motion DNA, we use a shared multilayer perceptron network to process each representative frame $\mathbf{\hat{T}}_j, j=0,1,...,\hat{N}$ and then apply average-pooling and an additional linear layer to obtain the final feature vector $w$. We concatenate $w$ at the end of each $z_t$ and use that as input to the decoder.   

To encourage the local motion generator to adopt the Motion DNA to generate variations without conflicting with the keyframe constraints, we design two losses to encourage the generator to place representative poses from the Motion DNA into the synthesized motion at suitable locations. 

The first loss $L^G_{DNA_1}$ encourages all of the representative poses to show up in the output sequence. For each representative frame $\mathbf{\hat{T}}_j$, we find the most similar frame in the synthesized motion $\mathbf{S}$ and compute the error $e_j$ between the pair. 
%\cyn{I am confused about that sentence you added. I thought the representative frames and synthesized frames you are comparing there have translation representation? Then why is there root rotation in there? }\yi{I explained below}
\begin{equation}
\begin{aligned}
\quad & L^G_{DNA_1} = 1/\hat{N} \sum_{j=0,..,\hat{N}} e_j
\quad & e_j = \min_{\mathbf{S}_i \in \mathbf{S}} ||\Lambda(\mathbf{S}_i) - \mathbf{\hat{T}}_j||^2_2
\end{aligned}
\label{eqt:DNA1}
\end{equation}
$\Lambda(\mathbf{S}_i)$ is the local pose of $\mathbf{S}_i$ without root rotation. Likewise, the representative poses $\mathbf{\hat{T}}_j$ also does not contain root rotations. In this way, we only care about the relative posture and not direction.

Because $L^G_{DNA_1}$ does not consider how the representative frames are distributed among the generated frames, it is possible that the representative poses all placed in a small time interval, which is not desirable. 
Therefore, we use a second loss $L^G_{DNA_2}$ to encourage the representative poses to be distributed  evenly throughout the entire synthesized sequence. 
Specifically, we cut the whole synthesized sequence at the keyframe points, and divide it into $K$ intervals, $u_k, k=0,1,...,K-1$, with each interval having the length of $N_k$, so $S = [S_{u_0}, S_{u_1}, ..., S_{u_{K-1}}]$. If $N_k$ is shorter than 3 seconds, we consider it is hard to place representative poses in it, otherwise we want the synthesized sub-sequence to contain frames that closely resemble $\hat{N}_k = \lfloor{N_k / 3}\rfloor$ input representative frames. In practice, for each frame $\mathbf{S}_{k,i}$ in $u_k$, we look for one of the representative poses in $\mathbf{\hat{T}}$ that is closest to it, and compute their error as $e'_{k,i}$. We consider the $\hat{N}_k$ frames with the lowest errors to be the frames where the representative poses should show up, and collect their errors. $L^G_{DNA_2}$ is defined as the average of those errors: 
\begin{equation}
\begin{aligned}
\quad & L^G_{DNA_2} = \frac{1}{\sum{\hat{N}_k}} \sum_{e'_{k,i}\in E'_k} e'_{k,i}
\\
\quad & e'_{k,i} = \min_{\mathbf{\hat{T}_j} \in \mathbf{\hat{T}}} ||\Lambda(\mathbf{S_{k,i}}) - \mathbf{\hat{T}}_j||^2_2
\end{aligned}
\label{eqt:DNA2}
\end{equation}
,$e'_{k,i}$ is the minimum error between the $i$-th local pose in the interval $u_k$ and all the representative frames. $E'_k$ is the set of the lowest $\hat{N}_k$ errors in the interval $u_k$. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Variation Generation}
%\label{sec:variations}

%Mention that the data in each sub catergory are not sufficient for training alone. 


%\yi{maybe I should delete this section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Sampling}

%\subsubsection{Sampling for Representative Frames and Motion DNA}
%min 128
%1 second (60 frames), max: 1 meter 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Post-processing}
\label{sec:post}
Though we use L2 reconstruction loss to enforce the keyframe constraints, the output sequence might not exactly match the input at keyframe locations. When needed, simple post processing can be applied to achieve exact keyframe matching~\cite{Harvey:2018:Recurrent}. 
%Although we punish the pose and root coordinate difference errors at the given frames during training, it is not guaranteed that the output sequence can perfectly match the given frames. 
%In cases that the users are strict about this, simple post processing can be applied to eliminate small difference errors. 
%We use the same interpolation method as in the Target Blend Section of \cite{Harvey:2018:Recurrent} to pull the synthetic motion strictly to the given keyframes. 
With small keyframe mismatches in our synthesized motion, the adjustments are nearly undetectable.
%With the small offset errors in our synthetic motion, the adjustment is nearly undetectable.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dataset and Training}
\label{sec:train_details}

We construct our training dataset based on the CMU Motion Capture Dataset \cite{cmu}. We only use motion clips in which the entire motion is performed on a flat plane. We automatically filtered out noisy frames (see appendix). The final dataset contains 79 classes of motion clips of length ranging from 4 seconds to 96 seconds. We use 1220 clips for training and 242 clips for testing.

For training, we first train the Global Path Predictor model (\sect{sec:global}), fix its weights and then train the Local Motion Generator model (\sect{sec:generation}). 
For each generator update, we update the discriminator once. 
We feed fixed-length 2048-frame sequences to the generator with a batch size of 4. We train the discriminator using 16 real sequences of length ranging from 256 to 1024 frames in each batch. We use the RMSprop optimizer with the default parameters from Pytorch~\cite{paszke2017automatic}. Other details about training parameters and frame sampling can be found in the Appendix. 








%\cyn{Yi, mention in a sentence or two how you sampled the representative frames used for motion DNA}

%Cynthia: No time to write this
%\subsubsection{Infinite Interval Inbetweening}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Cynthia: No time to write this
%\subsection{Inbetweening of extensive intervals}
%Extensive interval 


%\subsection{Discussion on Alternative Methods}
%RNN,
%Bidirectional RNN,
%Supervised Model,
%Most deep learning methods use the recurrent networks for generating motions (cite a,b,c,d), but it is hard to plot arbitrary number of future frames with their 


%Generate path first than local motion
%...

%We don't add a loss on the velocity because it will mess up with the adversarial loss 

%Input the output motion with the given frames to the discriminator will crash the network
%\cyn{Lower priority given time}

==> Long-term 3D Motion Inbetweening/related_work.tex <==
\section{Related Work}
There are many works in human motion synthesis using statistical, data-driven and physics-based methods~\cite{rose1998verbs, rose2001artist, kovar2004automated, grochow2004style, mukai2005geostatistical, LevineWHPK12, lee2002interactive, park2002line, safonova2007construction, likhachev2004ara, won2014generating, AllenF09, TanGLT14, LevineK14, MordatchLAPT15, peng2017deeploco, yu2018learning, jiang2019synthesis, liu2018learning, hong2019, naderi2017discovering, liu2017learning, peng2018deepmimic, lee2019scalable}. A comprehensive survey is beyond the scope of this work. We discuss more related papers below on transition synthesis, deep learning and biomechanic constraints.

\textbf{Transition Synthesis.} Statistical motion models have been used to generate transitions in human animations. Chai and Hodgins~\shortcite{ChaiH07} and Min~et~al.~\shortcite{MinCC09} developed MAP optimization frameworks, which can create transitions and also follow other constraints. Wang et~al.~\shortcite{WangFH08} use Gaussian process dynamical models to create transitions and synthesize motion. Lehrmann~et~al.~\shortcite{LehrmannGN14} use a nonlinear Markov model called a dynamic forest model to synthesize transitions and perform action recognition. Agrawal and van de Panne~\shortcite{agrawal2016task} develop a model for synthesizing complex locomotions including side steps, toe pivots, heel pivots, and foot slides, which allows task-specific locomotion to be produced. Harvey~and~Pal~\shortcite{Harvey:2018:Recurrent} use a recurrent network model based on long short-term memory (LSTM) to synthesize human locomotion, including for transitions. Unlike Harvey~and~Pal~\shortcite{Harvey:2018:Recurrent}, who train on a fixed interval of 60 frames for locomotion, our method can synthesize longer-term motions across different kinds of movement (e.g. walking, dance), can use a wide range of different temporal intervals between an arbitrary number of keyframes, and can provide a variety of outputs.  %, and more closely match the endpoint constraints. %Harvey and Pal \cite{Harvey:2018:Recurrent} showed promising results on synthesizing realistic transitions for loco-motions in an interval of 60 frames, however, their method performs badly on longer interval and more complex motions, cannot provide multiple transitions and is limited to perceiving only one future frame and without time information (the network is trained with fixed time gap), thus, not robust for inbetweening applications. % Siggraph 2018 Techinical Brief
%Recurrent transition networks for character locomotion~\cite{}
%(And the related works in this paper, Jimei's comment was to especially make sure to include the classic ones from Section 2.3)
%\cyn{Yi, is the last sentence true? Do we more closely match the endpoint constraints?}

%\textbf{Kernel-based Methods for Motion Synthesis.} Approaches using kernels such as radial basis functions (RBFs) and Gaussian process regression have been used for motion synthesis tasks. Rose~et~al. \shortcite{rose1998verbs} call parameterized motions such as walking and running ``verbs" and use RBFs and polynomials to blend between them. Rose et al. \shortcite{rose2001artist} use RBFs to perform interpolations of example motions and positions for inverse kinematics tasks. Kovar and Gleicher~\shortcite{kovar2004automated} create a search algorithm that can identify similar motions in a dataset and use them to create continuous motions by a similar blending procedure. Grochow~et~al.~\shortcite{grochow2004style} use Gaussian processes to perform inverse kinematics based on a dataset of human poses. Mukai and Kuriyama~\shortcite{mukai2005geostatistical} use   Gaussian process regression to better model correlations between motions, and also improve on artifacts in end effectors such as foot sliding.  Levine~et~al.~\shortcite{LevineWHPK12} use a Gaussian process latent variable model to perform animation and control tasks in a low-dimensional space. Unlike these works, our method can synthesize long-term transitions, and also is based on a deep generative adversarial architecture.

%\textbf{Motion Graph Methods for Motion Synthesis.} From an original dataset of motion clips, one can construct a motion graph where each state refers to a frame of pose and each edge represents the transition between two states. Given the start and end state, as well as the motion graph, the optimal path are searched to match the input constraints. However, the search space grows exponentially with the number of the edges. To prune the motion graph, Lee~et~al.~\shortcite{lee2002interactive} clustered similar states, and Park~et~al.~\shortcite{park2002line} and Safonova~et~al.~\shortcite{safonova2007construction} limited the transitions to states with contact changes. Safonova~et~al. further used an RAR*~\shortcite{likhachev2004ara} algorithm to speed up the search process which takes a few minutes to compute a close to optimal 15 second long motion from a database of 6-7 minutes of motion. However, their algorithm uses a heuristic function aiming for searching the shortest path between the start and end poses, and cannot be applied when the time interval is constrained. In contrast, our method is trained on over 2.5 million frames (around 6 hours) of motion clips and only takes 0.16 second to infer a 15 second long motion. Won~et~al.~\shortcite{won2014generating} use motion graphs to generate multi-character interaction scenes from high-level text descriptions, and rank these motions using  hand-crafted features.
%\yi{remember to fill the number}
%\textbf{Interactive Character Control.}


%\textbf{Neural Network Controllers for Physics-based Motion.} Neural network approaches have been used for motion controllers in physically-based animation. Allen and Faloutsos~\shortcite{AllenF09} evolve the topology of neural networks to allow for the creation of increasingly complicated motion behavior. Tan~et~al.~\shortcite{TanGLT14} apply this to the task of learning controllers for bicycle stunts. Levine and Vladlen \shortcite{LevineK14} use a neural network-based policy search to learn policies for complex tasks such as bipedal push recovery and walking on uneven terrain. Mordatch~et~al.~\shortcite{MordatchLAPT15} use a recurrent architecture to learn a controller for complex dynamic motions such as swimming, flying, and biped and quadruped walking. More recently, there has been a focus on locomotion, such as learning both low- and high-level controllers for locomotion~\cite{peng2017deeploco}, and achieving more realistic and symmetric~\cite{yu2018learning} or biologically plausible~\cite{jiang2019synthesis} locomotion. Networks have also been used recently to learn controllers from example motion clips in sports such as basketball~\cite{liu2018learning} and soccer~\cite{hong2019}. Naderi~et~al.~\shortcite{naderi2017discovering} also address path and movement planning for wall climbing humanoids. Reinforcement learning has been used recently to learn a variety of motions, such as  scheduling the order of a diverse array of ``control fragments" for a motion controller~\cite{liu2017learning} and learning a variety of skills by imitation such as acrobatics and martial arts~\cite{peng2018deepmimic}.  Lee~et~al.~\shortcite{lee2018interactive} use RNNs to learn interactive character controllers that model rich connections between different control objectives and a large repertoire of actions.  Lee~et~al.~\shortcite{lee2019scalable} develop a deep reinforcement learning approach to control a human musculoskeletal model containing 346 muscles using a two-level model that specifies skeletal motion in one level and muscle coordination in the other level. Our method can also be viewed as a multi-level model, where we model motion as two separate parts: local joint motion and global motion of the hip. Unlike these papers, we do not focus on physically-based animation, but instead synthesis of perceptually plausible motions: these can be useful for applications such as games or movie scenes where physicality is not a strict requirement.

% Text from paper ``A Deep Learning Framework for Character Motion Synthesis and Editing." Connelly rewrote it above.
%Allen and Faloutsos [2009] use the
%NEAT algorithm, that evolves the topology of the neural network
%for controlling bipedal characters. Tan et al. [2014] apply this technique for control of bike stunts. Levine and Vladlen [2014] learn
%the optimal control policies using neural networks and apply it to
%bipedal gait control. Mordatch et al. [2015] apply a recurrent neural network (RNN) to learn a near-optimal feedback controller for
%articulated characters. 

\textbf{Deep Learning for Motion Synthesis.} Recently, researchers have investigated the use of deep learning approaches for synthesizing plausible but not necessarily physically correct motions. Holden~et~al.~\shortcite{holden2016deep} learn a motion manifold from a large motion capture dataset, and then learn a feedforward network that maps user goals such as a motion path to the motion manifold. 
Li~et~al.~\shortcite{li2017auto} introduced the first real-time method for synthesizing indefinite complex human motions using an auto-conditioned recurrent neural network, but only high-level motion styles can be provided as input.
Holden~et~al.~\shortcite{holden2017phase} later proposed a synthesis approach for character motions using a neural network structure that computes weights as cyclic functions of user inputs and the phase within the motion.
Zhang~et~al.~\shortcite{zhang2018mode} synthesize quadruped motion by dynamically blending groups of weights based on the state of the character. Aristidou~et~al.~\shortcite{aristidou2018deep} break motion sequences into motion words and then cluster these to find descriptive representations of the motion that are called motion signatures and motifs. In contrast, we focus here on synthesizing plausible long-term motion transitions.
Followed by the work of Cai~et~al. ~\shortcite{cai2018deep} which focuses on video completion, recently Yan~et~al.~\shortcite{yanconvolutional} proposed a convolution network that can transform random latent vectors from Gaussian process to human motion sequences, and demonstrated the ability to complete motion between disjoint short motion sequences. But their framework only generates and matches local motion without global motion, and does not apply to the cases of sparsely given individual keyframes. Moreover, they do not provide users explicit control on the style of output motion or consider the body flexibility constraints. We do not compare with their method because it does not provide open-sourced code. Zhang and van de Panne~\shortcite{zhang2018data} use a neural autoregressive model to interpolate between keyframes while following the style of the exemplar corpus. This is demonstrated for a lamp object, unlike our method, which focuses on human motion.  Wang~et~al.~\shortcite{wang2019spatio} focus on learning a deep motion manifold that is suitable for motion synthesis with a long time horizon and motion denoising, which is able to represent the modalities and variance of the motion. 

%Siggraph 2016:
%A Deep Learning Framework for Character Motion Synthesis and Editing~\cite{holden2016deep} (Jimei recommended to base related work on their related work)

%Phase-Functioned Neural Networks for Character Control~\cite{holden2017phase}

%Mode-Adaptive Neural Networks for Quadruped Motion Control~\cite{zhang2018mode}

%Siggraph Asia 2018:
%Deep Motifs and Motion %Signatures~\cite{aristidou2018deep}

\textbf{Joint Angle Limits and Forward Kinematics.} Recently, there has been research into the representation of joint angles and the use of forward kinematics within networks. Akhter and Black~\shortcite{akhter2015pose} learn a pose-dependent model of joint angle limits, which generalizes well but avoids impossible poses. Jiang and Liu~\shortcite{jiang2018data} use a physics simulation to accurately simulate human joint limits.  We are inspired by these works and represent local joint angles in a limited range in our network.  Villegas~et~al.~\shortcite{villegas2018neural} use a recurrent neural network with a forward kinematics layer to perform unsupervised motion retargeting. We similarly use a forward kinematics layer in our network. Pavllo~et~al.~\shortcite{pavllo2019} use a quaternionic representation for joint angles and a forward kinematics layer. Zhou~et~al.~\shortcite{zhou2019} showed recently that when the complete set of 3D rotations need to be represented, a 6D rotation representation often performs better: we therefore adopt that angle representation for the root node.


%Pose-Conditioned Joint Angle Limits for 3D Human Pose Reconstruction~\cite{akhter2015pose}

%Data-driven approach to simulating realistic human joint constraints~\cite{}

%Neural Kinematic Networks for Unsupervised Motion Retargeting~\cite{villegas2018neural}

%Modeling Human Motion with Quaternion-based Neural Networks~\cite{pavllo2019}
%
%On the Continuity of Rotation Representations in Neural Networks~\cite{zhou2019}





==> Long-term 3D Motion Inbetweening/table/eval_errros_per_DNA_rate.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Input \\ DNAs \\ rate(1/s)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Root\\ Error\\ (cm)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Local \\ PoseError\\ (cm)\end{tabular} & \begin{tabular}[c]{@{}l@{}}DNA \\ PoseError\\ (cm)\end{tabular} & \begin{tabular}[c]{@{}l@{}}DNA\\ Cover\\ (std)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Motion\\ Variance\\ (std)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Bad \\ Frames\\ (\%)\end{tabular} \\ \hline
1s                                                                 & 30.9                                                        & 3.6                                                               & 9.5                                                             & 0.30                                                        & {\color[HTML]{5682D6} 0.259}                                      & {\color[HTML]{3A70D9} 0.076}                                 \\ \hline
2s                                                                 & 33.9                                                        & 3.5                                                               & 9.4                                                             & 0.30                                                        & {\color[HTML]{3A70D9} 0.255}                                      & {\color[HTML]{5682D6} 0.096}                                 \\ \hline
\rowcolor[HTML]{F7F7D5} 
3s                                                                 & 31.8                                                        & 3.7                                                               & 9.9                                                             & 0.30                                                        & {\color[HTML]{1938B0} 0.248}                                      & {\color[HTML]{3A70D9} 0.074}                                 \\ \hline
4s                                                                 & 31.5                                                        & 3.6                                                               & 9.7                                                             & 0.30                                                        & {\color[HTML]{244FCA} 0.253}                                      & {\color[HTML]{244FCA} 0.065}                                 \\ \hline
5s                                                                 & 33.2                                                        & 3.6                                                               & 9.4                                                             & 0.29                                                        & {\color[HTML]{1938B0} 0.250}                                      & {\color[HTML]{1938B0} 0.060}                                 \\ \hline
6s                                                                 & 30.6                                                        & 3.6                                                               & 9.7                                                             & 0.29                                                        & {\color[HTML]{233578} 0.245}                                      & {\color[HTML]{233578} 0.052}                                 \\ \hline
7s                                                                 & 30.8                                                        & 3.6                                                               & 9.5                                                             & 0.29                                                        & {\color[HTML]{010163} 0.241}                                      & {\color[HTML]{010163} 0.045}                                 \\ \hline
8s                                                                 & 28.7                                                        & 3.6                                                               & 9.7                                                             & 0.27                                                        & 0.233                                                             & {\color[HTML]{333333} 0.037}                                 \\ \hline
\end{tabular}
\caption{Errors with different input DNA rates.}
\label{tab:errors_per_DNArate}
\end{table}

==> Long-term 3D Motion Inbetweening/table/eval_key_errors.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|r|}{Raw Keyframe Root Error} & 10.0 cm & Raw Keyframe Local Pose Error  & 3.5 cm \\ \hline
Post Keyframe Root Error                      &         & Post Keyframe Local Pose Error &        \\ \hline
DNA Pose Error\_1                             & 8.4 cm  & DNA Pose Error\_2              & 6.5 cm \\ \hline
\end{tabular}
\caption{Mean Keyframe Matching Errors of GTN}
\label{tab:key_errors}
\end{table}

==> Long-term 3D Motion Inbetweening/table/eval_path_prediction.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
$V_{1}$ & $V_{2}$ & $V_{4}$ & $V_{8}$ & $V_{16}$ & $V_{32}$ & $V_{64}$ & $V_{128}$ & Y   \\ \hline
0.7  & 0.8  & 1.1  & 1.5  & 1.9   & 2.8   & 3.9   & 5.5    & 1.8 \\ \hline
\end{tabular}
\caption{Global path prediction mean errors in centimeters. $V_n$ is the mean error of the root (hip) translation differences in the x-z plane for poses predicted at $n$ frames in the future. $Y$ is the mean error of the root (hip) along the y axis.}
\label{tab:hip_prediction_error}
\end{table}

==> Long-term 3D Motion Inbetweening/table/eval_representation.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
                                                                        & Mean(cm) & Max(cm) & Std(cm) \\ \hline
Quaternion                                                                    & 9.03     & 179.66  & 16.33   \\ \hline
Vanilla Euler Angles                                                          & 2.7      & 48.7    & 2.1     \\ \hline
\begin{tabular}[c]{@{}l@{}}Range-Constrained\\ Euler + 6D root (Ours)\end{tabular} & 2.3      & 34.9    & 1.5     \\ \hline
\end{tabular}
\caption{IK Reconstruction errors using different rotation representations. The quaternion and vanilla Euler angle representations are used for all nodes. Ours uses the range-constrained Euler representation for non-root nodes and the continuous 6D representation~\cite{zhou2019} for the root node.}
\label{tab:RP}
\end{table}

==> Long-term 3D Motion Inbetweening/table/eval_speed.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
Sequence Length (frames) & \begin{tabular}[c]{@{}l@{}}512\\ (8 s)\end{tabular} & \begin{tabular}[c]{@{}l@{}}1024\\ (17 s)\end{tabular} & \begin{tabular}[c]{@{}l@{}}2048\\ (34 s)\end{tabular} & \begin{tabular}[c]{@{}l@{}}4096\\ (68 s)\end{tabular} \\ \hline
Local Motion Generation (s)      & 0.019       & 0.023         & 0.021                & 0.022              \\ \hline
Global Path Prediction (s)      & 0.033       & 0.061          & 0.131                 & 0.237              \\ \hline
Post-processing (s)       & 0.008             & 0.017          & 0.036                 & 0.070                                                  \\ \hline
Total (s)                & 0.059             & 0.101         & 0.188                  & 0.329                                                  \\ \hline
\end{tabular}
\caption{Mean Computation Time for Generating Different Lengths of Motions. s refers to second.  }
\label{tab:speed}
\end{table}

==> Long-term 3D Motion Inbetweening/table/networks.tex <==
\begin{table*}[]
\small\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{llllllll}
\multicolumn{8}{l}{Encoder}                                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{Layer}      & \multicolumn{1}{l|}{in\_ch} & \multicolumn{1}{l|}{out\_ch}  & \multicolumn{1}{l|}{kernel size} & \multicolumn{1}{l|}{stride} & \multicolumn{1}{l|}{pad} & \multicolumn{1}{l|}{ratio} & \multicolumn{1}{l|}{out\_len} \\ \hline
\multicolumn{1}{|l|}{res\_1}     & \multicolumn{1}{l|}{3M+3M}  & \multicolumn{1}{l|}{384}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/1}        & \multicolumn{1}{l|}{N/2}      \\ \hline
\multicolumn{1}{|l|}{res\_2}     & \multicolumn{1}{l|}{384}    & \multicolumn{1}{l|}{384}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/2}        & \multicolumn{1}{l|}{N/4}      \\ \hline
\multicolumn{1}{|l|}{res\_3}     & \multicolumn{1}{l|}{384}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/3}        & \multicolumn{1}{l|}{N/8}      \\ \hline
\multicolumn{1}{|l|}{res\_4}     & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/4}        & \multicolumn{1}{l|}{N/16}     \\ \hline
\multicolumn{1}{|l|}{res\_5}     & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{768}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/5}        & \multicolumn{1}{l|}{N/32}     \\ \hline
\multicolumn{1}{|l|}{res\_6}     & \multicolumn{1}{l|}{768}    & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/6}        & \multicolumn{1}{l|}{N/64}     \\ \hline
\multicolumn{8}{l}{Motion DNA Encoder}                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{conv\_1}    & \multicolumn{1}{l|}{3(M-1)} & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{0}   & \multicolumn{1}{l|}{-}          & \multicolumn{1}{l|}{$\hat{N}$}        \\ \hline
\multicolumn{1}{|l|}{affine} & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{$\hat{N}$}        \\ \hline
\multicolumn{1}{|l|}{CPReLU}     & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{$\hat{N}$}        \\ \hline
\multicolumn{1}{|l|}{conv\_2}    & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{$\hat{N}$}        \\ \hline
\multicolumn{1}{|l|}{affine} & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{$\hat{N}$}        \\ \hline
\multicolumn{1}{|l|}{AvgPool}    & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{1}        \\ \hline
\multicolumn{8}{l}{Decoder}                                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{res\_1}     & \multicolumn{1}{l|}{2048}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{0}   & \multicolumn{1}{l|}{1/1}        & \multicolumn{1}{l|}{N/64}     \\ \hline
\multicolumn{1}{|l|}{res\_2}     & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/1.4}      & \multicolumn{1}{l|}{N/64}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_3}  & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/1.6}      & \multicolumn{1}{l|}{N/32}     \\ \hline
\multicolumn{1}{|l|}{res\_4}     & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{768}      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/2.2}      & \multicolumn{1}{l|}{N/32}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_5}  & \multicolumn{1}{l|}{768}    & \multicolumn{1}{l|}{768}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1.0/2.8}    & \multicolumn{1}{l|}{N/16}     \\ \hline
\multicolumn{1}{|l|}{res\_6}     & \multicolumn{1}{l|}{768}    & \multicolumn{1}{l|}{768}      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1.0/3.6}    & \multicolumn{1}{l|}{N/16}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_7}  & \multicolumn{1}{l|}{768}    & \multicolumn{1}{l|}{768}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1.0/4.6}    & \multicolumn{1}{l|}{N/8}      \\ \hline
\multicolumn{1}{|l|}{res\_8}     & \multicolumn{1}{l|}{768}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/5.8}      & \multicolumn{1}{l|}{N/8}      \\ \hline
\multicolumn{1}{|l|}{res\_t\_9}  & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/7.2}      & \multicolumn{1}{l|}{N/4}      \\ \hline
\multicolumn{1}{|l|}{res\_10}    & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/8.8}      & \multicolumn{1}{l|}{N/4}      \\ \hline
\multicolumn{1}{|l|}{res\_t\_11} & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/10.6}     & \multicolumn{1}{l|}{N/2}      \\ \hline
\multicolumn{1}{|l|}{res\_12}    & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/12.6}     & \multicolumn{1}{l|}{N/2}      \\ \hline
\multicolumn{1}{|l|}{res\_t\_13} & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/14.8}     & \multicolumn{1}{l|}{N}        \\ \hline
\multicolumn{1}{|l|}{res\_14}    & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{6+3(M-1)} & \multicolumn{1}{l|}{3}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/17.2}     & \multicolumn{1}{l|}{N}        \\ \hline
\multicolumn{8}{l}{Discriminator}                                                                                                                                                                                                                       \\ \hline
\multicolumn{1}{|l|}{res\_1}     & \multicolumn{1}{l|}{3(M-1)} & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/1}        & \multicolumn{1}{l|}{N/2}      \\ \hline
\multicolumn{1}{|l|}{res\_2}     & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/2}        & \multicolumn{1}{l|}{N/4}      \\ \hline
\multicolumn{1}{|l|}{res\_3}     & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/3}        & \multicolumn{1}{l|}{N/8}      \\ \hline
\multicolumn{1}{|l|}{res\_4}     & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{512}      & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/4}        & \multicolumn{1}{l|}{N/16}     \\ \hline
\multicolumn{1}{|l|}{res\_5}     & \multicolumn{1}{l|}{512}    & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/5}        & \multicolumn{1}{l|}{N/32}     \\ \hline
\multicolumn{1}{|l|}{res\_6}     & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1024}     & \multicolumn{1}{l|}{4}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{1}   & \multicolumn{1}{l|}{1/6}        & \multicolumn{1}{l|}{N/64}     \\ \hline
\multicolumn{1}{|l|}{conv\_7}    & \multicolumn{1}{l|}{1024}   & \multicolumn{1}{l|}{1}        & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{0}   & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{N/64}     \\ \hline


\multicolumn{8}{l}{Global Path Predictor}                                                                                                                                                                                                                       \\ \hline
\multicolumn{1}{|l|}{res\_1}     & \multicolumn{1}{l|}{3(M-1)} & \multicolumn{1}{l|}{128}      & \multicolumn{1}{l|}{12}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{5}   & \multicolumn{1}{l|}{1/1}        & \multicolumn{1}{l|}{N/2}      \\ \hline
\multicolumn{1}{|l|}{res\_2}     & \multicolumn{1}{l|}{128}    & \multicolumn{1}{l|}{128}      & \multicolumn{1}{l|}{12}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{5}   & \multicolumn{1}{l|}{1/2}        & \multicolumn{1}{l|}{N/4}      \\ \hline
\multicolumn{1}{|l|}{res\_3}     & \multicolumn{1}{l|}{128}    & \multicolumn{1}{l|}{256}      & \multicolumn{1}{l|}{12}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{5}   & \multicolumn{1}{l|}{1/3}        & \multicolumn{1}{l|}{N/8}      \\ \hline
\multicolumn{1}{|l|}{res\_4}     & \multicolumn{1}{l|}{256}    & \multicolumn{1}{l|}{256}      & \multicolumn{1}{l|}{12}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{5}   & \multicolumn{1}{l|}{1/4}        & \multicolumn{1}{l|}{N/16}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_5}     & \multicolumn{1}{l|}{256}    & \multicolumn{1}{l|}{256}     & \multicolumn{1}{l|}{8}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{3}   & \multicolumn{1}{l|}{1/5}        & \multicolumn{1}{l|}{N/8}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_6}     & \multicolumn{1}{l|}{256}   & \multicolumn{1}{l|}{256}     & \multicolumn{1}{l|}{8}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{3}   & \multicolumn{1}{l|}{1/6}        & \multicolumn{1}{l|}{N/4}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_7}    & \multicolumn{1}{l|}{256}   & \multicolumn{1}{l|}{128}        & \multicolumn{1}{l|}{8}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{3}   & \multicolumn{1}{l|}{1/7}           & \multicolumn{1}{l|}{N/2}     \\ \hline
\multicolumn{1}{|l|}{res\_t\_8}    & \multicolumn{1}{l|}{128}   & \multicolumn{1}{l|}{128}        & \multicolumn{1}{l|}{8}      & \multicolumn{1}{l|}{2}      & \multicolumn{1}{l|}{3}   & \multicolumn{1}{l|}{1/8}           & \multicolumn{1}{l|}{N}     \\ \hline
\multicolumn{1}{|l|}{res\_9}    & \multicolumn{1}{l|}{128}   & \multicolumn{1}{l|}{3}        & \multicolumn{1}{l|}{5}      & \multicolumn{1}{l|}{1}      & \multicolumn{1}{l|}{2}   & \multicolumn{1}{l|}{1/9}           & \multicolumn{1}{l|}{N}     \\ \hline
\end{tabular}
\caption{Network Architectures. res indicates the 1D residual convolution layer. res\_t refers to the 1-D transpose residual convolution layer. in\_ch is the input channel number, out\_ch is the output channel number, ratio is the residual ratio defined in \sect{sec:generation} and out\_len is the output sequence length of each layer. }
\label{tab:network_architectures}
\end{table*}

==> Long-term 3D Motion Inbetweening/table/rotation_range.tex <==
\begin{table*}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
Joint         & x range   & y range   & z range   & Order & Joint        & x range   & y range  & z range  & Order \\ \hline
hip           & -360, 360 & -360, 360 & -360, 360 & xzy   & lCollar      & -30, 30   & -30, 30  & -10, 10  & xzy   \\ \hline
abdomen       & -45, 68   & -30, 30   & -45, 45   & xzy   & lShldr       & -90, 135  & -110, 30 & -70, 60  & xzy   \\ \hline
chest         & -45, 45   & -30, 30   & -45, 45   & xzy   & lForeArm     & 0, 0      & 0, 150   & -30, 120 & yxz   \\ \hline
neck          & -37, 22   & -30, 30   & -45, 45   & xzy   & lHand        & -90, 90   & -20, 30  & 0, 0     & xzy   \\ \hline
head          & -37, 22   & -30, 30   & -45, 45   & xzy   & lThumb1      & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
leftEye       & 0, 0      & 0, 0      & 0, 0      & xzy   & lThumb2      & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
leftEye\_Nub  & -         & -         & -         & xzy   & lThumb\_Nub  & -         & -        & -        & xzy   \\ \hline
rightEye      & 0, 0      & 0, 0      & 0, 0      & xzy   & lIndex1      & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rightEye\_Nub & -         & -         & -         & xzy   & lIndex2      & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rCollar       & -30, 30   & -30, 30   & -10, 10   & xzy   & lIndex2\_Nub & -         & -        & -        & xzy   \\ \hline
rShldr        & -90, 135  & -30, 110  & -70, 60   & xzy   & lMid1        & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rForeArm      & 0, 0      & 0, 150    & -30, 120  & yxz   & lMid2        & 0, 0      & 0, 0     & 0, 0     & yxz   \\ \hline
rHand         & -90, 90   & -30, 20   & 0, 0      & xzy   & lMid\_Nub    & -         & -        & -        & xzy   \\ \hline
rThumb1       & 0, 0      & 0, 0      & 0, 0      & xzy   & lRing1       & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rThumb2       & 0, 0      & 0, 0      & 0, 0      & xzy   & lRing2       & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rThumb\_Nub   & -         & -         & -         & xzy   & lRing\_Nub   & -         & -        & -        & xzy   \\ \hline
rIndex1       & 0, 0      & 0, 0      & 0, 0      & xzy   & lPinky1      & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rIndex2       & 0, 0      & 0, 0      & 0, 0      & xzy   & lPinky2      & 0, 0      & 0, 0     & 0, 0     & xzy   \\ \hline
rIndex2\_Nub  & -         & -         & -         & xzy   & lPinky\_Nub  & -         & -        & -        & xzy   \\ \hline
rMid1         & 0, 0      & 0, 0      & 0, 0      & xzy   & rButtock     & -20, 20   & -20, 20  & -10, 10  & xzy   \\ \hline
rMid2         & 0, 0      & 0, 0      & 0, 0      & xzy   & rThigh       & -180, 100 & -180, 90 & -60, 70  & xzy   \\ \hline
rMid\_Nub     & -         & -         & -         & xzy   & rShin        & 0, 170    & 0, 0     & 0, 0     & xzy   \\ \hline
rRing1        & 0, 0      & 0, 0      & 0, 0      & xzy   & rFoot        & -31, 63   & -30, 30  & -20, 20  & xzy   \\ \hline
rRing2        & 0, 0      & 0, 0      & 0, 0      & xzy   & rFoot\_Nub   & -         & -        & -        & xzy   \\ \hline
rRing\_Nub    & -         & -         & -         & xzy   & lButtock     & -20, 20   & -20, 20  & -10, 10  & xzy   \\ \hline
rPinky1       & 0, 0      & 0, 0      & 0, 0      & xzy   & lThigh       & -180, 100 & -180, 90 & -60, 70  & xzy   \\ \hline
rPinky2       & 0, 0      & 0, 0      & 0, 0      & xzy   & lShin        & 0, 170    & 0, 0     & 0, 0     & xzy   \\ \hline
rPinky\_Nub   & -         & -         & -         & xzy   & lFoot        & -31, 63   & -30, 30  & -20, 20  & xzy   \\ \hline
              &           &           &           & xzy   & lFoot\_Nub   & -         & -        & -        & xzy   \\ \hline
\end{tabular}
\caption{Range and order of the rotations at each joint defined in the CMU Motion Capture Dataset. Note that finger motions are not captured in this dataset.}
\label{tab:rotation}
\end{table*}

==> Long-term 3D Motion Inbetweening/table/user_study_result.tex <==
\begin{table}[]
\small
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{User Study}                                                                                                                     \\ \hline
                                                                 & \multicolumn{3}{c|}{\textbf{Ours}} & \multicolumn{2}{c|}{\textbf{RTN}} \\ \hline
Train Setting                                                    & \multicolumn{3}{c|}{All-Random}               & Walk-1s          & All-4s         \\ \hline
Test Setting                                                     & All-Random       & Walk-1s      & All-4s      & Walk-1s          & All-4s         \\ \hline
Real                                                      & 193              & 216          & 217         & 156              & 314            \\ \hline
Synthetic                                                 & 124              & 94           & 163         & 154              & 9              \\ \hline
\begin{tabular}[c]{@{}l@{}}User Preference \end{tabular} & 39.1\%           & 30.3\%       & 42.9\%      & 49\%             & 2.8\%          \\ \hline
Margin of Error                                                  & $\pm$5.4\%           & $\pm$5.1\%       & $\pm$5.0\%      & $\pm$5.6\%           & $\pm$1.8\%         \\ \hline
\multicolumn{6}{|c|}{Input frame Alignment Error}                                                                                                       \\ \hline
Joint Error (cm)                                            & 3.5              & 4.4          & 5.6         & 2.3              & 30.3           \\ \hline
Root Error (cm)                                             & 10.0             & 5.1          & 4.5         & 10.7             & 155.4          \\ \hline
\end{tabular}
\caption{Evaluation results for motion quality and keyframe alignment. The first four rows of numbers are the user study results collected from 101 human workers. The rows ``real" and ``synthetic" are the number of workers who chose the real or synthetic motions, respectively. ``User preference" is the percentage of synthetic motions  chosen out of total pairs, and the margins of error are listed on the next row with confidence level at 95\%. The last two rows are the mean Euclidean error of the global root positions and the local joint positions of the input keyframes. Please refer to \sect{sect:rtn_comparison} for the definitions of the training and test settings.}
\label{tab:user_study_results}
\end{table}

==> table/eval_errros_per_DNA_rate.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Input \\ DNAs \\ rate(1/s)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Root\\ Error\\ (cm)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Local \\ PoseError\\ (cm)\end{tabular} & \begin{tabular}[c]{@{}l@{}}DNA \\ PoseError\\ (cm)\end{tabular} & \begin{tabular}[c]{@{}l@{}}DNA\\ Cover\\ (std)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Motion\\ Variance\\ (std)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Bad \\ Frames\\ (\%)\end{tabular} \\ \hline
1s                                                                 & 30.9                                                        & 3.6                                                               & 9.5                                                             & 0.30                                                        & {\color[HTML]{5682D6} 0.259}                                      & {\color[HTML]{3A70D9} 0.076}                                 \\ \hline
2s                                                                 & 33.9                                                        & 3.5                                                               & 9.4                                                             & 0.30                                                        & {\color[HTML]{3A70D9} 0.255}                                      & {\color[HTML]{5682D6} 0.096}                                 \\ \hline
\rowcolor[HTML]{F7F7D5} 
3s                                                                 & 31.8                                                        & 3.7                                                               & 9.9                                                             & 0.30                                                        & {\color[HTML]{1938B0} 0.248}                                      & {\color[HTML]{3A70D9} 0.074}                                 \\ \hline
4s                                                                 & 31.5                                                        & 3.6                                                               & 9.7                                                             & 0.30                                                        & {\color[HTML]{244FCA} 0.253}                                      & {\color[HTML]{244FCA} 0.065}                                 \\ \hline
5s                                                                 & 33.2                                                        & 3.6                                                               & 9.4                                                             & 0.29                                                        & {\color[HTML]{1938B0} 0.250}                                      & {\color[HTML]{1938B0} 0.060}                                 \\ \hline
6s                                                                 & 30.6                                                        & 3.6                                                               & 9.7                                                             & 0.29                                                        & {\color[HTML]{233578} 0.245}                                      & {\color[HTML]{233578} 0.052}                                 \\ \hline
7s                                                                 & 30.8                                                        & 3.6                                                               & 9.5                                                             & 0.29                                                        & {\color[HTML]{010163} 0.241}                                      & {\color[HTML]{010163} 0.045}                                 \\ \hline
8s                                                                 & 28.7                                                        & 3.6                                                               & 9.7                                                             & 0.27                                                        & 0.233                                                             & {\color[HTML]{333333} 0.037}                                 \\ \hline
\end{tabular}
\caption{Errors with different input DNA rates.}
\label{tab:errors_per_DNArate}
\end{table}

==> table/eval_key_errors.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|r|}{Raw Keyframe Root Error} & 10.0 cm & Raw Keyframe Local Pose Error  & 3.5 cm \\ \hline
Post Keyframe Root Error                      &         & Post Keyframe Local Pose Error &        \\ \hline
DNA Pose Error\_1                             & 8.4 cm  & DNA Pose Error\_2              & 6.5 cm \\ \hline
\end{tabular}
\caption{Mean Keyframe Matching Errors of GTN}
\label{tab:key_errors}
\end{table}
